Dispatching to Parallel Servers: Solutions of Poisson's Equation for First-Policy Improvement

Policy iteration techniques for multiple-server dispatching rely on the computation of value functions. In this context, we consider the continuous-space M/G/1-FCFS queue endowed with an arbitrarily-designed cost function for the waiting times of the incoming jobs. The associated relative value function is a solution of Poisson's equation for Markov chains, which in this work we solve in the Laplace transform domain by considering an ancillary, underlying stochastic process extended to (imaginary) negative backlog states. This construction enables us to issue closed-form relative value functions for polynomial and exponential cost functions and for piecewise compositions of the latter, in turn permitting the derivation of interval bounds for the relative value function in the form of power series or trigonometric sums. We review various cost approximation schemes and assess the convergence of the interval bounds these induce on the relative value function. Namely: Taylor expansions (divergent, except for a narrow class of entire functions with low orders of growth), and uniform approximation schemes (polynomials, trigonometric), which achieve optimal convergence rates over finite intervals. This study addresses all the steps to implementing dispatching policies for systems of parallel servers, from the specification of general cost functions towards the computation of interval bounds for the relative value functions and the exact implementation of the first-policy improvement step.

==> QUESTA20_macros.tex <==
\newcommand{\valuefunction}{v} % !
\newcommand{\purevaluefunction}{w} % !
\newcommand{\costfunction}{c} % !
\newcommand{\varmeancost}{\varsigma} % !
\newcommand{\specialmatrixfunction}{y} % !
\newcommand{\uppertriangular}{M} % !
\newcommand{\specialmatrix}{Y} % !


\renewcommand{\valuefunction}{v} % !
\renewcommand{\purevaluefunction}{c} % !
\renewcommand{\costfunction}{f} % !
\renewcommand{\varmeancost}{\varsigma} % !
\renewcommand{\specialmatrixfunction}{w} % !
\renewcommand{\uppertriangular}{X} % !
\renewcommand{\specialmatrix}{W} % !

\newcommand{\nocolsep}{\arraycolsep=1.4pt\def\arraystretch{1}}

%\renewcommand{\eqref}[1]{\noeqref{#1}\text{(}\ref{#1}\text{)}}%\!\!


\let\oldnl\nl% Store \nl in \oldnl
\newcommand{\nonl}{\renewcommand{\nl}{\let\nl\oldnl}}% Remove line number for one line

\newcommand{\horizontalline}{\noindent\makebox[\linewidth]{\rule{\columnwidth}{0.4pt}}\\ }

\def\smallint{\begingroup\textstyle \int\endgroup}



\makeatletter
\newlength\@SizeOfCirc%
\newcommand{\cwArrow}[1]{%
\setlength{\@SizeOfCirc}{5pt}%
\tikz [x=1.0ex,y=1.0ex,line width=.24ex, draw=black]%
\draw [->,>=stealth,anchor=center]%
(0,-0.2\@SizeOfCirc) -- (0,1.0\@SizeOfCirc) arc (90:-90:1.0\@SizeOfCirc);%
}%
\newcommand{\ccwArrow}[1]{%
\setlength{\@SizeOfCirc}{5pt}%
\tikz [x=1.0ex,y=1.0ex,line width=.24ex, draw=black]%
\draw [->,>=stealth,anchor=center]%
(0,-0.2\@SizeOfCirc) -- (0,1.0\@SizeOfCirc) arc (90:270:1.0\@SizeOfCirc);%
}%
\makeatother

\newcommand{\setst}{\, | \,}


\DeclareMathOperator\spanset{span}
\newcommand{\spanx}[1]{\spanset(#1)}

 \newcommand{\defeq}{:=}

\def\quad{\hskip1em\relax}
\def\qquad{\hskip2em\relax}

\newcommand{\lnx}[1]{\ln(#1)}
\newcommand{\Lnx}[1]{\ln\left(#1\right)}

\newcommand{\makenindex}[2]{{#1}^{(#2)}}
\newcommand{\dmakenindex}[2]{{#1}^{(#2)\prime}}

\newcommand{\diracfunction}{\delta}
\newcommand{\dirack}[1]{\diracfunction\lbrack{#1}\rbrack}
\newcommand{\diract}[1]{\diracfunction({#1})}

%\newcommand{\radius}{\rho}
\newcommand{\radiussing}[1]{\radius_{#1}}
\newcommand{\cut}{\underline{\sing}}
\newcommand{\truecut}{\underline{\tilde{\sing}}}

\newcommand{\modulus}[1]{|#1|}
\newcommand{\bigmodulus}[1]{\big|#1\big|}
\newcommand{\Modulus}[1]{\left|#1\right|}
\newcommand{\norm}[1]{\|#1\|}
\newcommand{\Norm}[1]{\left\|#1\right\|}
\newcommand{\invnorm}[1]{\|#1\|_\star}
\newcommand{\invNorm}[1]{\left\|#1\right\|_\star}
\newcommand{\normi}[2]{\norm{#1}_{#2}}
\newcommand{\Normi}[2]{\Norm{#1}_{#2}}



\newcommand{\tricomifunction}{\Psi}
\newcommand{\Tricomi}[3]{\tricomifunction\left(#1,#2,#3\right)}
\newcommand{\tricomi}[3]{\tricomifunction(#1,#2,#3)}
\newcommand{\errorfunction}{\textup{erf}}
\newcommand{\Error}[1]{\errorfunction\left({#1}\right)}
\newcommand{\error}[1]{\errorfunction(#1)}

\newcommand{\incompletegammafunction}{\Upgamma}
\newcommand{\incompletegamma}[2]{\incompletegammafunction(#1,#2)}
\newcommand{\Incompletegamma}[2]{\incompletegammafunction\left(#1,#2\right)}
\newcommand{\gammafunction}{\Upgamma}
\newcommand{\gammax}[1]{\gammafunction(#1)}
\newcommand{\Gammax}[1]{\gammafunction\left(#1\right)}

\newcommand{\order}{n}
\newcommand{\kind}{k}
\newcommand{\lind}{l}
\newcommand{\orderi}[1]{\order_{#1}}
\newcommand{\errfunction}{\eta}
\newcommand{\errifunction}[1]{\errfunction_{#1}}
\newcommand{\errn}[1]{\makenindex{\errfunction}{#1}}
\newcommand{\Excset}{\Xi}%{\Upxi}
\newcommand{\excfunction}{\xi}
\newcommand{\excx}[1]{\excfunction(#1)}
\newcommand{\lexcfunction}{\excfunction_-}
\newcommand{\lexcx}[1]{\lexcfunction(#1)}
\newcommand{\uexcfunction}{\excfunction_+}
\newcommand{\uexcx}[1]{\uexcfunction(#1)}
\newcommand{\excifunction}[1]{\excfunction_{#1}}
\newcommand{\excit}[2]{\excifunction{#1}(#2)}
\newcommand{\decisionset}{\sigma}

\newcommand{\period}{\taufunction}
\newcommand{\periodcostfunction}{\tilde\costfunction}
\newcommand{\periodcostx}[1]{\periodcostfunction(#1)}
\newcommand{\mirrorcostfunction}{\check \costfunction}
\newcommand{\mirrorcostx}[1]{\mirrorcostfunction(#1)}
\newcommand{\thetacostfunction}{\tilde \costfunction}
\newcommand{\thetacostx}[1]{\thetacostfunction(#1)}
\newcommand{\blthetafunction}{\tilde{\bl}}
\newcommand{\bltheta}[1]{\blthetafunction(#1)}
\newcommand{\bigbltheta}[1]{\blthetafunction\big(#1\big)}
\newcommand{\Bltheta}[1]{\blthetafunction\left(#1\right)}
\newcommand{\dblthetafunction}{\blthetafunction^\prime}
\newcommand{\dbltheta}[1]{\dblthetafunction(#1)}
\newcommand{\fouriercoef}{\tilde{\alpha}}%{\alpha}
\newcommand{\fouriercoefk}[1]{\fouriercoef_{#1}}
\newcommand{\mirrorfouriercoef}{\check{\alpha}}
\newcommand{\mirrorfouriercoefk}[1]{\mirrorfouriercoef_{#1}}
\newcommand{\realfouriercoef}{\beta}
\newcommand{\realfouriercoefk}[1]{\realfouriercoef_{#1}}
\newcommand{\bernsteinfunction}{b}
\newcommand{\bernsteinnfunction}[1]{\bernsteinfunction^{(#1)}}
\newcommand{\bernsteinnx}[2]{\bernsteinnfunction{#1}{(#2)}}
\newcommand{\tsfunction}{t}
\newcommand{\tsnfunction}[1]{\tsfunction^{(#1)}}
\newcommand{\tsnx}[2]{\tsnfunction{#1}{(#2)}}
\newcommand{\mirroritsfunction}{\check\tsfunction}
\newcommand{\mirroritsnfunction}[1]{\mirroritsfunction^{(#1)}}
\newcommand{\mirroritsnx}[2]{\mirroritsnfunction{#1}{(#2)}}
\newcommand{\itsfunction}{\tilde\tsfunction}
\newcommand{\itsnfunction}[1]{\itsfunction^{(#1)}}
\newcommand{\itsnx}[2]{\itsnfunction{#1}{(#2)}}
\newcommand{\itscoef}{\varrho}%{\rho}
\newcommand{\itscoefnk}[2]{\itscoef_{#1,#2}}
\newcommand{\ptsfunction}{\hat\tsfunction}
\newcommand{\ptsnfunction}[1]{\ptsfunction^{(#1)}}
\newcommand{\ptsnx}[2]{\ptsnfunction{#1}{(#2)}}
\newcommand{\blstar}{\bl^\star}
\newcommand{\deltastar}{\bl^\star}
\newcommand{\thetastar}{\theta^\star}
\newcommand{\xistar}{\xi^\star}
\newcommand{\npolydegree}{m}
\newcommand{\allpolycostfunction}{f}
\newcommand{\allpolycostnfunction}[1]{\allpolycostfunction_{#1}}
\newcommand{\allpolycostnx}[2]{\allpolycostnfunction{#1}(#2)}
\newcommand{\Allpolycostnx}[2]{\allpolycostnfunction{#1}\left(#2\right)}
\newcommand{\polyphifunction}{\phi}
%\newcommand{\polyphinfunction}[1]{\polyphifunction_{#1}}
%\newcommand{\polyphinlambx}[3]{\polyphinfunction{#1}(#2,#3)}
%\newcommand{\Polyphinlambx}[3]{\polyphinfunction{#1}\left(#2,#3\right)}
\newcommand{\polyphinlambfunction}[2]{\polyphifunction_{#1,#2}}
\newcommand{\polyphinlambx}[3]{\polyphinlambfunction{#1}{#2}(#3)}
\newcommand{\Polyphinlambx}[3]{\polyphinlambfunction{#1}{#2}\left(#3\right)}
\newcommand{\dqallpolycostnfunction}[2]{\allpolycostfunction^{(#2)}_{#1}}
\newcommand{\dqallpolycostnx}[3]{\dqallpolycostnfunction{#1}{#2}(#3)}
\newcommand{\dqAllpolycostnx}[3]{\dqallpolycostnfunction{#1}{#2}\left(#3\right)}
\newcommand{\npolycostfunction}{g}
\newcommand{\npolycostnfunction}[1]{\npolycostfunction_{#1}}
\newcommand{\npolycostnx}[2]{\npolycostnfunction{#1}(#2)}
\newcommand{\Npolycostnx}[2]{\npolycosntfunction{#1}\left(#2\right)}
\newcommand{\dpolydegree}{n}
\newcommand{\dpolycostfunction}{h}
\newcommand{\dpolycostnfunction}[1]{\dpolycostfunction_{#1}}
\newcommand{\dpolycostnx}[2]{\dpolycostnfunction{#1}(#2)}\newcommand{\Dpolycostnx}[2]{\dpolycostnfunction{#1}\left(#2\right)}
\newcommand{\integralk}[1]{\gamma_{#1}}
\newcommand{\integralklamb}[2]{\integralk{#1}(#2)}
\newcommand{\polylamb}{\altcomplex}
\newcommand{\realfouriercoefklamb}[2]{\hat{\alpha}_{#1}(#2)}
\newcommand{\polydegree}{l}
\newcommand{\polydegreek}[1]{\polydegree({#1})}
\newcommand{\intbound}[2]{\kappa(#1,#2)}
\newcommand{\irrationalfunction}{\varpi}%{\mu}
\newcommand{\dnirrationalfunction}[1]{\irrationalfunction^{(#1)}}
\newcommand{\irrationalx}[1]{\irrationalfunction(#1)}
\newcommand{\dnirrationalx}[2]{\dnirrationalfunction{#1}(#2)}
\newcommand{\anglesingtau}[2]{\theta(#1,#2)}
\newcommand{\evenoddcoef}{\kappa}
\newcommand{\evencoef}{\evenoddcoef_\textup{e}}
\newcommand{\evencoefsingtauq}[3]{\evencoef(#1,#2;#3)}
\newcommand{\oddcoef}{\evenoddcoef_\textup{o}}
\newcommand{\oddcoefsingtauq}[3]{\oddcoef(#1,#2;#3)}
%\newcommand{\evenoddcoefksingtauq}[4]{\evenoddcoef(#1,#2,#3;#4)}
\newcommand{\evenoddcoefksingtauq}[4]{\evenoddcoef(#1,#3,#4)}


\newcommand{\polynomialcoeffunction}{\varsigma}
\newcommand{\polynomialcoef}[2]{\polynomialcoeffunction_{#1,#2}}
\newcommand{\bernsteincoeffunction}{\beta}
\newcommand{\bernsteincoef}[2]{\bernsteincoeffunction_{#1,#2}}
\newcommand{\bernsteinderivfunction}[2]{\hat\costfunction_{#1}^{(#2)}}
\newcommand{\bernsteinderivx}[3]{\bernsteinderivfunction{#1}{#2}(#3)}
\newcommand{\continuitymodulusfunction}{\omega}
\newcommand{\continuitymodulusSfunction}[1]{\continuitymodulusfunction}%{\continuitymodulusfunction_{#1}}
\newcommand{\continuitymodulusx}[1]{\continuitymodulusfunction(#1)}
\newcommand{\bigcontinuitymodulusx}[1]{\continuitymodulusfunction\big(#1\big)}
\newcommand{\Continuitymodulusx}[1]{\continuitymodulusfunction\left(#1\right)}
\newcommand{\continuitymodulusfx}[2]{\continuitymodulusSfunction(#1;#2)}
\newcommand{\bigcontinuitymodulusfx}[2]{\continuitymodulusSfunction\big(#1;#2\big)}
\newcommand{\Continuitymodulusfx}[2]{\continuitymodulusSfunction\left(#1;#2\right)}
\newcommand{\continuitymodulusSx}[2]{\continuitymodulusSfunction{#1}(#2)}
\newcommand{\ContinuitymodulusSx}[2]{\continuitymodulusSfunction{#1}\left(#2\right)}
\newcommand{\continuitymodulusSfx}[3]{\continuitymodulusSfunction{#1}(#2;#3)}
\newcommand{\ContinuitymodulusSfx}[3]{\continuitymodulusSfunction{#1}\left(#2;#3\right)}
\newcommand{\inflexionpoint}{\bl^\star}
\newcommand{\Lipschitz}{L}
\newcommand{\hoeldernconstant}{h}
\newcommand{\hoeldernexponent}{\alpha}
\newcommand{\continuitymodulussIfx}[4]{\continuitymodulusSfunction{#1}(#3;#2;#4)}
\newcommand{\bigcontinuitymodulussIfx}[4]{\continuitymodulusSfunction{#1}\big(#3;#2;#4\big)}
\newcommand{\ContinuitymodulussIfx}[4]{\continuitymodulusSfunction{#1}\left(#3;#2;#4\right)}
\newcommand{\coscoeffunction}{\nu}
\newcommand{\coscoef}[2]{\coscoeffunction(#1,#2)}
\newcommand{\Coscoef}[2]{\coscoeffunction\left(#1,#2\right)}
\newcommand{\polcoscoeffunction}{\gamma}%{\varrho}
\newcommand{\polcoscoef}[2]{\polcoscoeffunction(#1,#2)}
\newcommand{\translatedpolcoscoeffunction}{\bar\polcoscoeffunction}
\newcommand{\translatedpolcoscoef}[2]{\translatedpolcoscoeffunction(#1,#2)}
\newcommand{\funnyset}[2]{\bar\sigma(#1,#2)}
\newcommand{\taylorcoef}[2]{\alpha_{#2}(#1)}
\newcommand{\Taylorcoef}[2]{\alpha_{#2}\left(#1\right)}
\newcommand{\laurentcoef}[1]{\zeta_{#1}}

\newcommand{\exponentialdistri}[1]{\textup{Exp}({#1})}
\newcommand{\categoricaldistri}[1]{\textup{Cat}({#1})}
\newcommand{\MDPfunction}{\Phi}
\newcommand{\MDP}[1]{\MDPfunction_{#1}}
\newcommand{\MDPpolicyfunction}[1]{\MDPfunction^{#1}}
\newcommand{\MDPpolicy}[2]{\MDPpolicyfunction{#1}_{#2}}
\newcommand{\MDPkernelfunction}{P}
\newcommand{\MDPkernelifunction}[1]{\MDPkernelfunction_{#1}}
\newcommand{\MDPkernel}[2]{\MDPkernelfunction({#1},#2)}
\newcommand{\MDPkerneli}[3]{\MDPkernelifunction{#1}(#2,#3)}
\newcommand{\MDPkernelarfunction}[1]{\MDPkernelfunction^{\scalebox{0.8}{\scriptsize$(#1)$}}}
\newcommand{\MDPkernelar}[3]{\MDPkernelarfunction{#1}(#2,#3)}
\newcommand{\makeDE}[1]{\hat{#1}}%
\newcommand{\makeU}[1]{\widehat{#1}}%\widehat
\newcommand{\UMDPkernelfunction}{\makeU{\MDPkernelfunction}}
\newcommand{\UMDPkernel}[2]{\UMDPkernelfunction({#1},#2)}
\newcommand{\dMDPkernelfunction}{\MDPkernelfunction-\UMDPkernelfunction}
\newcommand{\dMDPkernel}[2]{(\dMDPkernelfunction)({#1},#2)}
\newcommand{\MDPspace}{\Omega}%{\mathcal{S}}
\newcommand{\MDPsubspace}{\genericset}
\newcommand{\MDPblsubspace}{\genericblset}
\newcommand{\MDPstsubspace}{\genericstset}
\newcommand{\solutionkernelfunction}{\Gamma}
\newcommand{\solutionkernelifunction}[1]{\solutionkernelfunction_{#1}}
\newcommand{\solutionkernel}[2]{\solutionkernelfunction({#1},#2)}
\newcommand{\Ucostfunction}{\makeU\costfunction}
\newcommand{\Ucostx}[1]{\Ucostfunction(#1)}
\newcommand{\Ucostxy}[2]{\Ucostfunction({#1},#2)}
\newcommand{\UDeltafunction}{\Updelta}%{h}%{\Delta}%{h}
\newcommand{\UDeltax}[1]{\UDeltafunction(#1)}
\newcommand{\Kquantity}{\kappa}%{K}
\newcommand{\alphafactor}{\alpha}
\newcommand{\nearonefunction}{\eta}
\newcommand{\nearones}[1]{\nearonefunction(#1)}
\newcommand{\jump}{\varepsilon}%{\nu}%{\upsilon}%{h}%{\Updelta}%{\gamma}
\newcommand{\Ujump}{\jump}%{\makeU{\jump}}%{h}%{\Updelta}%{\gamma}
\newcommand{\Ujumpi}[1]{\Ujump_{#1}}
\newcommand{\DEjump}{\makeDE{\jump}}%{h}%{\DEpdelta}%{\gamma}
\newcommand{\DEjumpi}[1]{\DEjump_{#1}}


\newcommand{\initialpolicyfunction}{\pi}
\newcommand{\initialpolicy}[1]{\initialpolicyfunction_{#1}}
\newcommand{\initialpolicyxy}[2]{\initialpolicyfunction(#1,#2)}
\newcommand{\initialpolicys}[1]{\initialpolicyfunction(#1)}
\newcommand{\osipolicyfunction}{\pi}
\newcommand{\osipolicyxy}[2]{\osipolicyfunction(#1,#2)}
\newcommand{\osipolicyx}[1]{\osipolicyfunction(#1)}
\newcommand{\probai}[1]{p_{#1}}
\newcommand{\osipolicyn}[1]{\osipolicyfunction^{(#1)}}
\newcommand{\osipolicynx}[2]{\osipolicyn{#1}{(#2)}}
%\newcommand{\valuenfunction}[1]{\valuefunction^{(#1)}}
%\newcommand{\valuenx}[2]{\valuenfunction{#1}{(#2)}}
\newcommand{\varmeancostn}[1]{\varmeancost^{(#1)}}
\newcommand{\varmeancosti}[1]{\varmeancost_{#1}}
\newcommand{\newpolicyfunction}{\hat{\osipolicyfunction}}
\newcommand{\newpolicyx}[1]{\newpolicyfunction{(#1)}}



\newcommand{\cosx}[1]{\cos(#1)}
\newcommand{\bigcosx}[1]{\cos\big(#1\big)}
\newcommand{\Cosx}[1]{\cos\left(#1\right)}
\newcommand{\cosnx}[2]{\cos^{#1}(#2)}
\newcommand{\bigcosnx}[2]{\cos^{#1}\big(#2\big)}
\newcommand{\Cosnx}[2]{\cos^{#1}\left(#2\right)} 
\newcommand{\Cossquaredx}[1]{\cos^2\left(#1\right)}
\newcommand{\arcosx}[1]{\cos^{-1}(#1)}
\newcommand{\arCosx}[1]{\cos^{-1}\left(#1\right)}
\newcommand{\atan}{\tan^{-1}}
\newcommand{\atanx}[1]{\atan(#1)}
\newcommand{\Atanx}[1]{\atan\left(#1\right)}
\newcommand{\acot}{\cot^{-1}}
\newcommand{\acotx}[1]{\acot(#1)}
\newcommand{\Acotx}[1]{\acot\left(#1\right)}
\newcommand{\sinx}[1]{\sin(#1)}
\newcommand{\bigsinx}[1]{\sin\big(#1\big)}
\newcommand{\Sinx}[1]{\sin\left(#1\right)}
\newcommand{\sinnx}[2]{\sin^{#1}(#2)}
\newcommand{\Sinnx}[2]{\sn^{#1}\left(#2\right)}
\newcommand{\Sinsquaredx}[1]{\sin^2\left(#1\right)}
\newcommand{\arctgx}[1]{\arctan(#1)}
\newcommand{\polcosnfunction}[1]{p_{#1}}
\newcommand{\polcosnx}[2]{\polcosnfunction{#1}(#2)}
\newcommand{\Polcosnx}[2]{\polcosnfunction{#1}\left(#2\right)}

\newcommand{\Gfunction}{G}
\newcommand{\Gpd}[2]{\Gfunction(#1,#2)}

\newcommand{\kronecker}[2]{\delta_{{#1}{#2}}}
\newcommand{\Kronecker}[2]{\delta_{{#1},{#2}}}

\newcommand{\ceil}[1]{\lceil#1\rceil}
\newcommand{\Ceil}[1]{\left\lceil#1\right\rceil}
\newcommand{\floor}[1]{\lfloor#1\rfloor}
\newcommand{\Floor}[1]{\left\lfloor#1\right\rfloor}

%\newcommand{\binomialcoef}[2]{\textup{\tiny{$\left(\!\begin{array}{c} #1 \\ #2 \end{array}\!\right)$}}}
\newcommand{\binomialcoef}[2]{\left({}^{#1}_{#2}\right)}
\newcommand{\Binomialcoef}[2]{\left({}^{#1}_{#2}\right)}
\newcommand{\bigbinomialcoef}[2]{\big({}^{#1}_{#2}\big)}
\newcommand{\Bigbinomialcoef}[2]{\Big(\nocolsep\begin{array}{c}{#1}\\{#2}\end{array}\Big)}


\newcommand{\scenariosfunction}{\phi}
\newcommand{\scenarios}[2]{\scenariosfunction(#1,#2)}
\newcommand{\Scenarios}[2]{\scenariosfunction\left(#1,#2\right)}
\newcommand{\normscenariosfunction}{\varphi}
\newcommand{\normscenarios}[2]{\normscenariosfunction(#1,#2)}
\newcommand{\normScenarios}[2]{\normscenariosfunction\left(#1,#2\right)}
\newcommand{\scenariosshapefunction}[1]{\vartheta^{(#1)}}
\newcommand{\scenariosshape}[3]{\scenariosshapefunction{#1}(#2,#3)}
\newcommand{\Scenariosshape}[3]{\scenariosshapefunction{#1}\left(#2,#3\right)}

\newcommand{\arrivalsetfunction}{S}
\newcommand{\arrivalset}[2]{\arrivalsetfunction(#1,#2)}

\newcommand{\timei}[1]{t_{#1}}

\newcommand{\altvaluezero}{g_0}
\newcommand{\picarda}{a}
\newcommand{\picardaprime}{\hat{a}}
\newcommand{\picardb}{b}
\newcommand{\picardL}{l}
\newcommand{\picardM}{m}
\newcommand{\picardaprimebis}{\tilde{\picarda}}
\newcommand{\picardcsti}[1]{\nu_{#1}}
\newcommand{\picardxi}[1]{\bl_{#1}}
\newcommand{\altvaluefunction}{\tilde{\valuefunction}}
\newcommand{\altvaluecst}{\nu_0}
\newcommand{\altdistricst}{\gamma_0}
\newcommand{\altvaluex}[1]{\altvaluefunction(#1)}
\newcommand{\altpurevaluefunction}{\tilde{\purevaluefunction}}
\newcommand{\altpurevaluex}[1]{\altpurevaluefunction(#1)}
\newcommand{\deltaaltvaluefunction}{\Delta\altvaluefunction}
\newcommand{\deltaaltvaluex}[1]{\deltaaltvaluefunction(#1)}
\newcommand{\deltaaltdistrifunction}{\Delta\altdistrifunction}
\newcommand{\deltaaltdistrix}[1]{\deltaaltdistrifunction(#1)}
\newcommand{\altvalueifunction}[1]{\altvaluefunction_{ #1}}
\newcommand{\altvalueix}[2]{\altvalueifunction{#1}(#2)}
\newcommand{\altvaluekfunction}[1]{\altvaluefunction^{(#1)}}
\newcommand{\altvaluekx}[2]{\altvaluekfunction{#1}(#2)}
\newcommand{\altpurevaluekfunction}[1]{\altpurevaluefunction^{(#1)}}
\newcommand{\altpurevaluekx}[2]{\altvaluekfunction{#1}(#2)}
\newcommand{\normset}{\mathcal{V}}
\newcommand{\invnormset}{\mathcal{F}}
\newcommand{\picardoperatorfunction}{\Gamma}
\newcommand{\picardoperator}[1]{\picardoperatorfunction_{#1}}
\newcommand{\picardoperatorf}[2]{\picardoperator{#1}{#2}}
\newcommand{\picardoperatorfx}[3]{\left(\picardoperatorf{#1}{#2}\right)(#3)}

\newcommand{\operatorfunction}{\partial}
\newcommand{\operator}[1]{\operatorfunction_{#1}}
\newcommand{\operatorf}[2]{\operator{#1}{#2}}
\newcommand{\operatorfx}[3]{\left(\operatorf{#1}{#2}\right)(#3)}


\newcommand{\projection}[1]{\lbrack{#1}\rbrack^+}
\newcommand{\sizedprojection}[2]{#1\lbrack{#2}#1\rbrack^+}
\newcommand{\Projection}[1]{\left\lbrack{#1}\right\rbrack^+}
\newcommand{\valuex}[1]{\valuefunction(#1)}
\newcommand{\valuesfunction}[1]{\makeserver{\valuefunction}{#1}}
\newcommand{\valuesx}[2]{\valuesfunction{#1}(#2)}
\newcommand{\valuecfunction}[1]{\makeclass{\valuefunction}{#1}}
\newcommand{\valuecx}[2]{\valuecfunction{#1}(#2)}
\newcommand{\valuezerofunction}{\valuefunction_0}
\newcommand{\valuezerox}[1]{\valuezerofunction(#1)}
\newcommand{\valuezerocfunction}[1]{\makeclass{\valuezerofunction}{#1}}
\newcommand{\valuezerocx}[2]{\valuezerocfunction{#1}(#2)}
\newcommand{\valueafunction}[1]{\valuefunction_{#1}}%{\tilde{\valuefunction}_{#1}}
\newcommand{\valueax}[2]{\valueafunction{#1}(#2)}
\newcommand{\purevalueafunction}[1]{\purevaluefunction_{#1}}%\tilde{\purevaluefunction}_{#1}}
\newcommand{\purevalueax}[2]{\purevalueafunction{#1}(#2)}
\newcommand{\dpurevalueafunction}[1]{\purevaluefunction^\prime_{#1}}
\newcommand{\dpurevalueax}[2]{\dpurevalueafunction{#1}(#2)}
\newcommand{\altvalueafunction}[1]{\hat{\valuefunction}_{#1}}
\newcommand{\altvalueax}[2]{\altvalueafunction{#1}(#2)}
\newcommand{\purealtvalueafunction}[1]{\hat{\purevaluefunction}_{#1}}
\newcommand{\purealtvalueax}[2]{\purealtvalueafunction{#1}(#2)}
\newcommand{\boundvaluefunction}{\bar\valuefunction}
\newcommand{\boundvaluex}[1]{\boundvaluefunction(#1)}
\newcommand{\boundpurevaluefunction}{\bar\purevaluefunction}
\newcommand{\boundpurevaluex}[1]{\boundpurevaluefunction(#1)}
\newcommand{\purevaluex}[1]{\purevaluefunction(#1)}
\newcommand{\purevaluenfunction}[1]{\makenindex{\purevaluefunction}{#1}}
\newcommand{\dpurevaluenfunction}[1]{\dmakenindex{\purevaluefunction}{#1}}
\newcommand{\purevaluenx}[2]{\purevaluenfunction{#1}(#2)}
\newcommand{\pureValuex}[1]{\purevaluefunction\left(#1\right)}
\newcommand{\pureValuenx}[2]{\purevaluenfunction{#1}\left(#2\right)}
\newcommand{\dpurevaluenx}[2]{\dpurevaluenfunction{#1}(#2)}
\newcommand{\dpureValuex}[1]{\dpurevaluefunction\left(#1\right)}
\newcommand{\dpureValuenx}[2]{\dpurepicavaluenfunction{#1}\left(#2\right)}
%\newcommand{\purevalueanfunction}[2]{\purevaluefunction_{#1}^{(#2)}}
%\newcommand{\dpurevalueanfunction}[2]{\dmakenindex{\purevalueafunction{#1}}{#2}}
\newcommand{\purevalueanfunction}[2]{\purevaluefunction_{#1:#2}}
\newcommand{\dpurevalueanfunction}[2]{\purevalueanfunction{#1}{#2}^\prime}
\newcommand{\purevalueanx}[3]{\purevalueanfunction{#1}{#2}(#3)}
\newcommand{\pureValueanx}[3]{\purevalueanfunction{#1}{#2}\left(#3\right)}
\newcommand{\dpurevalueanx}[3]{\dpurevalueanfunction{#1}{#2}(#3)}
\newcommand{\dpureValueanx}[3]{\dpurevalueanfunction{#1}{#2}\left(#3\right)}
\newcommand{\Uvaluefunction}{\makeU{\valuefunction}}%{\makeU\purevaluefunction}
\newcommand{\Uvaluex}[1]{\Uvaluefunction(#1)}
\newcommand{\Uvalueifunction}[1]{\Uvaluefunction_{#1}}
\newcommand{\Uvalueix}[2]{\Uvalueifunction{#1}(#2)}
\newcommand{\dUvaluefunction}{\Uvaluefunction^\prime}%{\makeU\purevaluefunction}
\newcommand{\dUvaluex}[1]{\dUvaluefunction(#1)}
\newcommand{\dUvalueifunction}[1]{\dUvaluefunction_{#1}}
\newcommand{\dUvalueix}[2]{\dUvalueifunction{#1}(#2)}
\newcommand{\Upurevaluefunction}{\makeU{\purevaluefunction}}%{\makeU\purevaluefunction}
\newcommand{\Upurevaluex}[1]{\Upurevaluefunction(#1)}
\newcommand{\dUpurevaluefunction}{\rightderivative\Upurevaluefunction}
\newcommand{\dUpurevaluex}[1]{\dUpurevaluefunction(#1)}
\newcommand{\DEvaluefunction}{\makeDE{\valuefunction}}%{\makeDE\purevaluefunction}
\newcommand{\DEvaluex}[1]{\DEvaluefunction(#1)}
\newcommand{\DEpurevaluefunction}{\makeDE{\purevaluefunction}}%{\makeDE\purevaluefunction}
\newcommand{\DEpurevaluex}[1]{\DEpurevaluefunction(#1)}
\newcommand{\dDEpurevaluefunction}{\rightderivative\DEvaluefunction}
\newcommand{\dDEpurevaluex}[1]{\dDEpurevaluefunction(#1)}
\newcommand{\costrate}{r}
\newcommand{\meancost}{\bar{\costfunction}}
\newcommand{\fixedcost}{h}
\newcommand{\dvaluefunction}{\valuefunction^\prime}
\newcommand{\dvaluex}[1]{\dvaluefunction(#1)}
\newcommand{\dpurevaluefunction}{\purevaluefunction^\prime}
\newcommand{\dpurevaluex}[1]{\dpurevaluefunction(#1)}
\newcommand{\dnpurevaluefunction}[1]{\purevaluefunction^{(#1)}}
\newcommand{\dnpurevaluex}[2]{\dnpurevaluefunction{#1}(#2)}
\newcommand{\dnpureValuex}[2]{\dnpurevaluefunction{#1}\left(#2\right)}
\newcommand{\Valuefunction}{V}
\newcommand{\Valuetfunction}[1]{\Valuefunction_{#1}}
\newcommand{\ValuetxT}[3]{\Valuetfunction{#1}(#2,#3)}
\newcommand{\st}{d}
\newcommand{\sts}[1]{\makeserver{\st}{#1}}
\newcommand{\nst}{A}
\newcommand{\shape}{q}
\newcommand{\strate}{\omega}
\newcommand{\stgrate}{\varsigma}
\newcommand{\knst}{a}
\newcommand{\pnst}{p}
\newcommand{\phnst}[1]{p^{[#1]}}
\newcommand{\pnstk}[1]{\pnst_{#1}}
\newcommand{\phnstk}[2]{\phnst{#1}_{#2}}
\newcommand{\bl}{u}
\newcommand{\bli}[1]{\bl_{#1}}
\newcommand{\blfunction}{U}
\newcommand{\blxt}[2]{\blfunction(#1,#2)}
\newcommand{\stochbl}{U}
\newcommand{\stochbli}[1]{\stochbl_{#1}}
\newcommand{\stochblk}[1]{\stochbl_{#1}}
\newcommand{\stochblik}[2]{\stochbl_{#1,#2}}
\newcommand{\stochblt}[1]{\stochbl({#1})}
\newcommand{\vari}{m}
\newcommand{\varix}[1]{\bar\vari(#1)}
\newcommand{\varbl}{\mu}
\newcommand{\bls}[1]{\bl_{#1}}
\newcommand{\altbl}{t}
\newcommand{\altaltbl}{t^\prime}
\newcommand{\altst}{y}
\newcommand{\stochst}{\st(\stoch)}
\newcommand{\stoch}{\omega}
\newcommand{\dl}{\tau}
\newcommand{\dlc}[1]{\makeclass{\dl}{#1}}
\newcommand{\stochdl}{\dl(\stoch)}
\newcommand{\truear}{\bar\lambda}
\newcommand{\ar}{\lambda}
\newcommand{\ari}[1]{\ar_{#1}}
\newcommand{\arc}[1]{\makeclass{\ar}{#1}}
\newcommand{\arprob}{p}
\newcommand{\probc}[1]{\makeclass{\arprob}{#1}}
\newcommand{\load}{\rho}
\newcommand{\loadi}[1]{\load_{#1}}
\newcommand{\loadzero}{\load_{0}}
\newcommand{\expectationfunction}{\mathbb{E}}
\newcommand{\expectation}[1]{\expectationfunction[#1]}
\newcommand{\condexpectation}[2]{\expectationfunction[#1|#2]}
\newcommand{\Expectation}[1]{\expectationfunction\left[#1\right]}
\newcommand{\bigexpectation}[1]{\expectationfunction\big[#1\big]}
\newcommand{\condExpectation}[2]{\expectationfunction\left[#1|#2\right]}
\newcommand{\condbigexpectation}[2]{\expectationfunction\big[#1|#2\big]}
\newcommand{\zero}[1]{o(#1)}
\newcommand{\Zero}[1]{o\left(#1\right)}
\newcommand{\magnitude}[1]{O(#1)}
\newcommand{\Magnitude}[1]{O\left(#1\right)}
\newcommand{\proba}[1]{\textup{Prob}(#1)}
\newcommand{\Proba}[1]{\textup{Prob}\left(#1\right)}
\newcommand{\one}[1]{\theta(#1)}
\newcommand{\ti}{t}
\newcommand{\ttt}{t_0}
\newcommand{\cost}{c}
\newcommand{\costc}[1]{\makeclass{\cost}{#1}}
\newcommand{\Cost}{H}
\newcommand{\Costc}[1]{\makeclass{\Cost}{#1}}
\newcommand{\costn}[1]{\costfunction[#1]}
\newcommand{\costx}[1]{\costfunction(#1)}
\newcommand{\costxy}[2]{\costfunction({#1},#2)}
\newcommand{\bigcostx}[1]{\costfunction\big(#1\big)}
\newcommand{\Costx}[1]{\costfunction\left(#1\right)}
\newcommand{\dcostfunction}{\costfunction^\prime}
\newcommand{\dcostx}[1]{\dcostfunction(#1)}
\newcommand{\dncostfunction}[1]{\costfunction^{(#1)}}
\newcommand{\dncostx}[2]{\dncostfunction{#1}(#2)}
\newcommand{\dnCostx}[2]{\dncostfunction{#1}\left(#2\right)}
\newcommand{\costafunction}[1]{\costfunction_{#1}}
\newcommand{\costax}[2]{\costafunction{#1}(#2)}
\newcommand{\altcostafunction}[1]{\hat{\costfunction}_{#1}}
\newcommand{\altcostax}[2]{\altcostafunction{#1}(#2)}
\newcommand{\Yset}{\mathcal{Y}}
\newcommand{\meancosta}[1]{\bar{\costfunction}_{#1}}
\newcommand{\meancosti}[1]{\bar{\costfunction}_{#1}}
\newcommand{\valuenfunction}[1]{\makenindex{\valuefunction}{#1}}
\newcommand{\valuenx}[2]{\valuenfunction{#1}(#2)}
\newcommand{\costnfunction}[1]{\makenindex{\costfunction}{#1}}%\varsigma
\newcommand{\costnx}[2]{\costnfunction{#1}(#2)}
%\newcommand{\costanfunction}[2]{\costafunction{#1}^{(#2)}}
%\newcommand{\costanfunction}[2]{\costafunction{#1:#2}}
\newcommand{\costanfunction}[2]{\costafunction{#1,#2}}
\newcommand{\costanx}[3]{\costanfunction{#1}{#2}(#3)}
\newcommand{\meancostn}[1]{\makenindex{\bar\costfunction}{#1}}
\newcommand{\event}{Y}
\newcommand{\deltat}{d t}
\newcommand{\coefdelta}{\alpha}
\newcommand{\altcoefdelta}{\beta}
\newcommand{\ceilm}{m}
\newcommand{\ceilmc}[1]{\makeclass{\ceilm}{#1}}
\newcommand{\delayfunction}{f_0}
\newcommand{\delayx}[1]{\delayfunction({#1})}
\newcommand{\stochdelayfunction}{F_0}
\newcommand{\stochdelayx}[1]{\stochdelayfunction({#1})}
\newcommand{\stochstzero}{\stochst_{0}}
\newcommand{\stzero}{\st_{0}}
\newcommand{\Wt}{W}
\newcommand{\trueWt}{\tilde{\Wt}}
\newcommand{\LSTstochstfunction}{\stochst^{\ast}}
\newcommand{\LSTstochsts}[1]{\LSTstochstfunction(#1)}
\newcommand{\LSTstochstzerofunction}{\stochstzero^{\ast}}
\newcommand{\LSTstochstzeros}[1]{\LSTstochstzerofunction(#1)}
\newcommand{\MaclaurinLSTstochstfunction}[1]{\hat\stochst^{\ast}_{#1}}
\newcommand{\MaclaurinLSTstochsts}[2]{\MaclaurinLSTstochstfunction{#1}(#2)}
\newcommand{\LSTWtfunction}{\Wt^{\ast}}
\newcommand{\LSTWts}[1]{\LSTWtfunction(#1)}
\newcommand{\LSTWTS}[1]{\LSTWtfunction\left(#1\right)}
\newcommand{\LSTtrueWtfunction}{\trueWt^{\ast}}
\newcommand{\LSTtrueWts}[1]{\LSTtrueWtfunction(#1)}
\newcommand{\LSThatWtfunction}{\hat\Wt^{\ast}}
\newcommand{\LSThatWts}[1]{\LSThatWtfunction(#1)}
\newcommand{\rightarc}{r}
\newcommand{\leftarc}{l}
\newcommand{\fLSTWtfunction}{\Wt^{\rightarc}}
\newcommand{\fLSTWtxs}[2]{\fLSTWtfunction(#1;#2)}
\newcommand{\fLSTWTXS}[2]{\fLSTWtfunction\left(#1;#2\right)}
\newcommand{\fLSTWtxfunction}[1]{\fLSTWtfunction_{#1}}
\newcommand{\fLSTWtlfunction}[1]{\fLSTWtfunction_{#1}}
\newcommand{\fLSTWtlxs}[3]{\fLSTWtlfunction{#1}(#2;#3)}
\newcommand{\fLSTWTlxs}[3]{\fLSTWtlfunction{#1}\left(#2;#3\right)}
\newcommand{\iLSTWtfunction}{\Wt^{\leftarc}}
\newcommand{\iLSTWtxs}[2]{\iLSTWtfunction(#1;#2)}
\newcommand{\iLSTWTXS}[2]{\iLSTWtfunction\left(#1;#2\right)}
\newcommand{\iLSTWtxfunction}[1]{\iLSTWtfunction_{#1}}
\newcommand{\iLSTWtlfunction}[1]{\iLSTWtfunction_{#1}}
\newcommand{\iLSTWtlxs}[3]{\iLSTWtlfunction{#1}(#2;#3)}
\newcommand{\iLSTWTlxs}[3]{\iLSTWtlfunction{#1}\left(#2;#3\right)}
\newcommand{\fraccst}{b}
\newcommand{\degfunction}{f}
\newcommand{\degfunctions}[1]{\degfunction(#1)}
\newcommand{\degfunctionn}[1]{\degfunction^{(#1)}}
\newcommand{\degfunctionns}[2]{\degfunctionn{#1}(#2)}
\newcommand{\dominantpole}{p}
\newcommand{\dominantpoleX}[1]{\dominantpole_{#1}}
\newcommand{\distrifunction}{F}
\newcommand{\distriXfunction}[1]{\distrifunction_{#1}}
\newcommand{\distriXx}[2]{\distriXfunction{#1}({#2})}
\newcommand{\deltadistrifunction}{\distrifunction^\Delta}
\newcommand{\discontinuities}{\mathcal{X}}
\newcommand{\deltadistriXfunction}[1]{\distrifunction^\Delta_{#1}}
\newcommand{\deltadistriXx}[2]{\deltadistriXfunction{#1}({#2})}
\newcommand{\ddeltadistrifunction}{\distrifunction^{\Delta\prime}}
\newcommand{\ddeltadistriXfunction}[1]{\distrifunction^{\Delta\prime}_{#1}}
\newcommand{\ddeltadistriXx}[2]{\ddeltadistriXfunction{#1}({#2})}
\newcommand{\altdistrifunction}{G}
\newcommand{\altdistrix}[1]{\altdistrifunction({#1})}
\newcommand{\altdistriifunction}[1]{\altdistrifunction_{#1}}
\newcommand{\altdistriix}[2]{\altdistriifunction{#1}({#2})}
\newcommand{\altdistrikfunction}[1]{\altdistrifunction^{(#1)}}
\newcommand{\altdistrikx}[2]{\altdistrikfunction{#1}({#2})}
\newcommand{\altddistrifunction}{\altdistrifunction^{\prime}}
\newcommand{\altddistrix}[1]{\altddistrifunction({#1})}
\newcommand{\discfunction}{J}
\newcommand{\discx}[1]{\discfunction({#1})}
\newcommand{\altaltdistrifunction}{H}
\newcommand{\altaltdistrix}[1]{\altaltdistrifunction({#1})}
\newcommand{\altaltddistrifunction}{\altaltdistrifunction^{\prime}}
\newcommand{\altaltddistrix}[1]{\altaltddistrifunction({#1})}
\newcommand{\invdistriXfunction}[1]{\distrifunction^{-1}_{#1}}
\newcommand{\invdistriXx}[2]{\invdistriXfunction{#1}({#2})}
\newcommand{\ddistrifunction}{\distrifunction^\prime}
\newcommand{\ddistriXfunction}[1]{\ddistrifunction_{#1}}
\newcommand{\invddistriXfunction}[1]{\distrifunction^{\prime-1}_{#1}}
\newcommand{\ddistriXx}[2]{\ddistriXfunction{#1}({#2})}
\newcommand{\invddistriXx}[2]{\invddistriXfunction{#1}({#2})}
\newcommand{\dddistrifunction}{\distrifunction^{\prime\prime}}
\newcommand{\dddistriXfunction}[1]{\dddistrifunction_{#1}}
\newcommand{\dddistriXx}[2]{\dddistriXfunction{#1}({#2})}
\newcommand{\reversedistrifunction}{\bar\distrifunction}
\newcommand{\reversedistriXfunction}[1]{\reversedistrifunction_{#1}}
\newcommand{\reversedistriXx}[2]{\reversedistriXfunction{#1}({#2})}
\newcommand{\sd}{d}%{\tilde{d}}



\newcommand{\makepurevffunction}{\mathcal{W}}
\newcommand{\makepurevf}[2]{\makepurevffunction(#1;#2)}
\newcommand{\Makepurevf}[2]{\makepurevffunction\left(#1;#2\right)}
\newcommand{\intervMakepurevf}[2]{\intervx\makepurevffunction\left(#1;#2\right)}

\newcommand{\pwcostifunction}[1]{\costfunction_{#1}}
\newcommand{\pwshiftedlaplaceifunction}[1]{\pwshiftedlaplacefunction_{#1}}
\newcommand{\pwshiftedlaplacest}[2]{\pwshiftedlaplacefunction({#1},{#2})}
\newcommand{\pwshiftedlaplaceist}[3]{\pwshiftedlaplaceifunction{#1}({#2},{#3})}
\newcommand{\pwcostix}[2]{\pwcostifunction{#1}(#2)}
\newcommand{\pwdeltafunction}{\Delta}
\newcommand{\pwdeltaifunction}[1]{\pwdeltafunction_{#1}}
\newcommand{\pwdeltax}[1]{\pwdeltafunction(#1)}
\newcommand{\pwdeltaix}[2]{\pwdeltaifunction{#1}(#2)}
\newcommand{\taufunction}{\tau}
\newcommand{\taui}[1]{\taufunction_{#1}}
\newcommand{\pwn}{h}
\newcommand{\barblfunction}{\bar{\bl}}
\newcommand{\barbli}[1]{\barblfunction_{#1}}
\newcommand{\pwKfunction}{K}
\newcommand{\pwKs}[1]{\pwKfunction(#1)}
\newcommand{\pwdnKfunction}[1]{\pwKfunction^{(#1)}}
\newcommand{\pwdnKs}[2]{\pwdnKfunction{#1}(#2)}
\newcommand{\pwyfunction}{g}
\newcommand{\pwynk}[2]{\pwyfunction({#1},{#2})}
\newcommand{\pwysumpmfunction}[1]{\pwysumfunction_{#1}}
\newcommand{\pwysumpmxs}[3]{\pwysumpmfunction{#1}(#2,#3)}
\newcommand{\pwfactors}[1]{\pwfactorfunction(#1)}
\newcommand{\pwfactorqfunction}[1]{\pwfactorfunction^{(#1)}}
\newcommand{\pwfactorqs}[2]{\pwfactorqfunction{#1}(#2)}
\newcommand{\degpwfactors}[1]{\degpwfactorfunction(#1)}
\newcommand{\degpwfactorqfunction}[1]{\degpwfactorfunction^{(#1)}}
\newcommand{\degpwfactorqs}[2]{\degpwfactorqfunction{#1}(#2)}
\newcommand{\pwchainmfunction}[1]{\pwchainfunction_{#1}}
\newcommand{\pwchainmqfunction}[2]{\pwchainmfunction{#1}^{(#2)}}
\newcommand{\pwchainmqs}[3]{\pwchainmqfunction{#1}{#2}(#3)}
\newcommand{\pwXchainmfunction}[1]{\pwXchainfunction_{#1}}
\newcommand{\pwXchainmqfunction}[2]{\pwXchainmfunction{#1}^{(#2)}}
\newcommand{\pwXchainmqp}[3]{\pwXchainmqfunction{#3:#1}{#2}}
\newcommand{\pwXprechainmfunction}[1]{\pwXprechainfunction_{#1}}
\newcommand{\pwXprechainmqfunction}[2]{\pwXprechainmfunction{#1}^{(#2)}}
\newcommand{\pwXprechainmqp}[3]{\pwXprechainmqfunction{#3:#1}{#2}}

\newcommand{\pwshiftedlaplacefunction}{\zeta}
\newcommand{\pwchainfunction}{\Psi}
\newcommand{\pwXchainfunction}{\Xi}
\newcommand{\pwXprechainfunction}{\bar\Xi}
\newcommand{\pwysumfunction}{\Lambda}
\newcommand{\pwfactorfunction}{\Upsilon}
\newcommand{\degpwfactorfunction}{\tilde\pwfactorfunction}
\newcommand{\pwkli}[2]{\kappa_{#1#2}}
\newcommand{\pwchifunction}{\chi}
\newcommand{\intpwchifunction}{\tilde{\pwchifunction}}
\newcommand{\pwchil}[1]{\pwchifunction_{#1}}
\newcommand{\degreefunction}{\nu}
\newcommand{\ResLSTWtpq}[2]{\varpi_{#1:#2}}
\newcommand{\iResLSTWtpq}[2]{\varpi^{\leftarc}_{#1:#2}}
\newcommand{\fResLSTWtpq}[2]{\varpi^{\rightarc}_{#1:#2}}
\newcommand{\pwvarphilj}[2]{\varphi_{{#1}{#2}}}
\newcommand{\ResLSTstochstpq}[2]{\xi_{#1:#2}}
\newcommand{\pwkout}{\bar\polynomialcoeffunction}
\newcommand{\pwnout}{k}
\newcommand{\pwkjin}[1]{\polynomialcoeffunction_{#1}}
\newcommand{\machinfunction}{\phi}
\newcommand{\machinstjm}[4]{\machinfunction_{#3,#4}({#1})}
\newcommand{\diffmachinfunction}{\Delta}
\newcommand{\diffmachinsm}[2]{\diffmachinfunction_{#2}({#1})}
\newcommand{\integratorfunction}{\tilde{\mu}}
\newcommand{\integratorqx}[2]{\integratorfunction^{(#1)}({#2})}


\newcommand{\pwNl}[1]{\bar{\nn}_{#1}}
\newcommand{\pwali}[2]{\sing_{#1#2}}
\newcommand{\pwnli}[2]{\nn_{#1#2}}
\newcommand{\pwchilstxm}[5]{\pwchil{#1}^{(#5)}(#2,#3,#4)}
\newcommand{\pwchisxm}[3]{\pwchifunction^{(#3)}(#1,#2)}
\newcommand{\intpwchisxm}[3]{\intpwchifunction^{(#3)}(#1,#2)}
\newcommand{\pole}{p}
\newcommand{\Pole}{\mathcal{P}}
\newcommand{\Polef}[1]{\Pole(#1)}
\newcommand{\iPole}{\Pole^{\leftarc}}
\newcommand{\fPole}{\Pole^{\rightarc}}
\newcommand{\iPolex}[1]{\iPole_{#1}}
\newcommand{\fPolex}[1]{\fPole_{#1}}
\newcommand{\degreep}[1]{\degreefunction({#1})}
\newcommand{\idegreefunction}{\degreefunction^{\leftarc}}
\newcommand{\idegreep}[1]{\idegreefunction({#1})}
\newcommand{\fdegreefunction}{\degreefunction^{\rightarc}}
\newcommand{\fdegreep}[1]{\fdegreefunction({#1})}
\newcommand{\pwvarphiljtxm}[5]{\pwvarphilj{#1}{#2}^{(#5)}(#3,#4)}
\newcommand{\weirdsumfunction}{\bar\sigma}
\newcommand{\weirdsum}[2]{\weirdsumfunction(#1,#2)}
\newcommand{\Weirdsum}[2]{\weirdsumfunction\left({#1},{#2}\right)}
\newcommand{\ROCfunction}{\textup{ROC}}
\newcommand{\ROC}[1]{\ROCfunction(#1)}


\newcommand{\trickfunction}{\tilde{m}}%{\mu}
\newcommand{\trickifunction}[1]{\trickfunction_{#1}}
\newcommand{\trickix}[2]{\trickifunction{#1}({#2})}
\newcommand{\trickx}[1]{\trickfunction({#1})}

\newcommand{\extvaluefunction}{\tilde\valuefunction}
\newcommand{\extvaluex}[1]{\extvaluefunction(#1)}
\newcommand{\extpurevaluefunction}{\tilde\purevaluefunction}
\newcommand{\extpurevaluex}[1]{\extpurevaluefunction(#1)}
\newcommand{\extdpurevaluefunction}{\rightderivative\extpurevaluefunction}%{\tilde\purevaluefunction^\prime}
\newcommand{\extdpurevaluex}[1]{\extdpurevaluefunction(#1)}


\newcommand{\makel}[1]{{#1}_{-}}
\newcommand{\makeu}[1]{{#1}_{+}}
\newcommand{\makelu}[1]{{#1}_{\mp}}

\newcommand{\deltak}[1]{\delta_{#1}}

\newcommand{\costderivativevector}{\tilde{\costfunction}}
\newcommand{\valuederivativevector}{\tilde{\purevaluefunction}}
\newcommand{\valueabsolutederivativevector}{\bar{\purevaluefunction}}
\newcommand{\valuemixedderivativevector}{\hat{\purevaluefunction}}
\newcommand{\impulsefunction}{\tilde{h}}%{\tilde{\zfunction}}
\newcommand{\invimpulsefunction}{\tilde{g}}
\newcommand{\costderivativevectorn}[1]{\costderivativevector^{(#1)}}
%\newcommand{\costderivativevectornk}[2]{\costderivativevectorn{#1}_{#2}} 
\newcommand{\costderivativevectornk}[2]{\costderivativevector_{#2}} 
\newcommand{\costderivativek}[1]{\costderivativevector_{#1}}
\newcommand{\valuederivativevectorn}[1]{\valuederivativevector^{(#1)}}
%\newcommand{\valuederivativevectornk}[2]{\valuederivativevectorn{#1}_{#2}} 
\newcommand{\valuederivativevectornk}[2]{\valuederivativevector_{#2}} 
\newcommand{\valuederivativek}[1]{\valuederivativevector_{#1}}
\newcommand{\valuederivativenk}[2]{\valuederivativevectorn{#1}_{#2}} 
\newcommand{\valueabsolutederivativek}[1]{\valueabsolutederivativevector_{#1}}
\newcommand{\valuemixedderivativek}[1]{\valuemixedderivativevector_{#1}}
\newcommand{\impulsex}[1]{\impulsefunction[#1]}
%\newcommand{\impulsex}[1]{\impulsefunction_{#1}}
\newcommand{\invimpulsex}[1]{\invimpulsefunction[#1]}
%\newcommand{\invimpulsex}[1]{\invimpulsefunction_{#1}}

\newcommand{\bound}{B}%{p}
\newcommand{\Rebound}{\bound_{\Re}}%{p}
\newcommand{\Imbound}{\bound_{\Im}}%{p}
\newcommand{\lbound}{\makel{b}}%{p}
\newcommand{\ubound}{\makeu{b}}%{q}
\newcommand{\lubound}{\makelu{b}}%{q}
\newcommand{\lmeancost}{\makel{\meancost}}%{p}
\newcommand{\umeancost}{\makeu{\meancost}}%{q}
\newcommand{\lumeancost}{\makelu{\meancost}}%{q}
\newcommand{\lcostfunction}{\makel{\costfunction}}%{p}
\newcommand{\lvaluefunction}{\makel{\valuefunction}}%{p}
\newcommand{\lpurevaluefunction}{\makel{\purevaluefunction}}%{p}
\newcommand{\ucostfunction}{\makeu{\costfunction}}%{q}
\newcommand{\uvaluefunction}{\makeu{\valuefunction}}%{q}
\newcommand{\upurevaluefunction}{\makeu{\purevaluefunction}}%{q}
\newcommand{\luvaluefunction}{\makelu{\valuefunction}}%{q}
\newcommand{\lupurevaluefunction}{\makelu{\purevaluefunction}}%{q}
\newcommand{\polycostfunction}{\hat\costfunction}
\newcommand{\polyvaluefunction}{\hat\valuefunction}
\newcommand{\polypurevaluefunction}{\hat\purevaluefunction}
\newcommand{\lpolycostfunction}{\makel{\polycostfunction}}
\newcommand{\upolycostfunction}{\makeu{\polycostfunction}}
\newcommand{\lupolycostfunction}{\makelu{\polycostfunction}}
\newcommand{\remaindercostfunction}{r}
\newcommand{\etax}[1]{\eta(#1)}
\newcommand{\xix}[1]{\xi(#1)}
\newcommand{\lvaluex}[1]{\lvaluefunction(#1)}%{p}
\newcommand{\uvaluex}[1]{\uvaluefunction(#1)}%{p}
\newcommand{\luvaluex}[1]{\luvaluefunction(#1)}%{p}
\newcommand{\lpurevaluex}[1]{\lpurevaluefunction(#1)}%{p}
\newcommand{\upurevaluex}[1]{\upurevaluefunction(#1)}%{p}
\newcommand{\lupurevaluex}[1]{\lupurevaluefunction(#1)}%{p}
\newcommand{\intervalfunction}{\Delta}
\newcommand{\intervalnfunction}[1]{\intervalfunction^{(#1)}}
\newcommand{\intervalx}[1]{\intervalfunction(#1)}
\newcommand{\intervalnx}[2]{\intervalnfunction{#1}(#2)}

\newcommand{\complexboundpurevaluefunction}{\varrho}
\newcommand{\complexboundpurevaluenfunction}[1]{\complexboundpurevaluefunction^{(#1)}}
\newcommand{\complexboundpurevaluenx}[2]{\complexboundpurevaluenfunction{#1}(#2)}

\newcommand{\intervx}[1]{[#1]}
\newcommand{\bigintervx}[1]{\big[#1\big]}
\newcommand{\Intervx}[1]{\left[#1\right]}
\newcommand{\realinterv}{\alpha}
\newcommand{\imaginaryinterv}{\beta}
\newcommand{\intervxy}[2]{\intervx{#1}(#2)}
\newcommand{\bigintervxy}[2]{\intervx{#1}\big(#2\big)}
\newcommand{\Intervxy}[2]{\Intervx{#1}(#2)}




\newcommand{\realintervn}[1]{\realinterv^{(#1)}}
\newcommand{\realintervnx}[2]{\realintervn{#1}(#2)}
\newcommand{\imaginaryintervn}[1]{\imaginaryinterv^{(#1)}}
\newcommand{\imaginaryintervnx}[2]{\imaginaryintervn{#1}(#2)}
\newcommand{\realintervi}[1]{\realinterv_{#1}}
\newcommand{\imaginaryintervi}[1]{\imaginaryinterv_{#1}}
\newcommand{\realintervni}[2]{\realintervn{#1}_{#2}}
\newcommand{\imaginaryintervni}[2]{\imaginaryintervn{#1}_{#2}}


\newcommand{\boundn}[1]{\makenindex{\bound}{#1}}%{p}
\newcommand{\Reboundn}[1]{\makenindex{\Rebound}{#1}}%{p}
\newcommand{\Imboundn}[1]{\makenindex{\Imbound}{#1}}%{p}
\newcommand{\lboundn}[1]{\makenindex{\lbound}{#1}}%{p}
\newcommand{\uboundn}[1]{\makenindex{\ubound}{#1}}%{p}
\newcommand{\luboundn}[1]{\makenindex{\lubound}{#1}}%{p}
\newcommand{\lmeancostn}[1]{\makenindex{\lmeancost}{#1}}%{p}
\newcommand{\umeancostn}[1]{\makenindex{\umeancost}{#1}}%{p}
\newcommand{\lumeancostn}[1]{\makenindex{\lumeancost}{#1}}%{p}
\newcommand{\lvaluenfunction}[1]{\makenindex{\lvaluefunction}{#1}}%{p}
\newcommand{\lpurevaluenfunction}[1]{\makenindex{\lpurevaluefunction}{#1}}%{p}
\newcommand{\uvaluenfunction}[1]{\makenindex{\uvaluefunction}{#1}}%{p}
\newcommand{\upurevaluenfunction}[1]{\makenindex{\upurevaluefunction}{#1}}%{p}
\newcommand{\luvaluenfunction}[1]{\makenindex{\luvaluefunction}{#1}}%{p}
\newcommand{\lupurevaluenfunction}[1]{\makenindex{\lupurevaluefunction}{#1}}%{p}
\newcommand{\polycostifunction}[1]{\polycostfunction_{#1}}
\newcommand{\polycostinfunction}[2]{\makenindex{\polycostifunction{#1}}{#2}}
\newcommand{\polycostnfunction}[1]{\makenindex{\polycostfunction}{#1}}
\newcommand{\lpolycostnfunction}[1]{\makenindex{\lpolycostfunction}{#1}}
\newcommand{\upolycostnfunction}[1]{\makenindex{\upolycostfunction}{#1}}
\newcommand{\lupolycostnfunction}[1]{\makenindex{\lupolycostfunction}{#1}}
\newcommand{\remaindercostnfunction}[1]{\makenindex{\remaindercostfunction}{#1}}
\newcommand{\polycostnx}[2]{\polycostnfunction{#1}(#2)}
\newcommand{\lpolycostnx}[2]{\lpolycostnfunction{#1}(#2)}
\newcommand{\upolycostnx}[2]{\upolycostnfunction{#1}(#2)}
\newcommand{\lupolycostnx}[2]{\lupolycostnfunction{#1}(#2)}
\newcommand{\polyvaluenfunction}[1]{\polyvaluefunction^{#1}}
\newcommand{\polyvaluenx}[2]{\polyvaluenfunction{#1}(#2)}
\newcommand{\polypurevaluenfunction}[1]{\polypurevaluefunction^{#1}}
\newcommand{\polypurevaluenx}[2]{\polypurevaluenfunction{#1}(#2)}
\newcommand{\remaindercostnx}[2]{\remaindercostnfunction{#1}(#2)}
\newcommand{\lvaluenx}[2]{\lvaluenfunction{#1}(#2)}%{p}
\newcommand{\uvaluenx}[2]{\uvaluenfunction{#1}(#2)}%{p}
\newcommand{\luvaluenx}[2]{\luvaluenfunction{#1}(#2)}%{p}
\newcommand{\lpurevaluenx}[2]{\lpurevaluenfunction{#1}(#2)}%{p}
\newcommand{\upurevaluenx}[2]{\upurevaluenfunction{#1}(#2)}%{p}
\newcommand{\lupurevaluenx}[2]{\lupurevaluenfunction{#1}(#2)}%{p}
\newcommand{\domainfunction}{\mathcal{V}}
\newcommand{\domainpsfunction}{\domainfunction^{\textup{P}}}
\newcommand{\domainps}[2]{\domainpsfunction_{#1}}
\newcommand{\domainffunction}{\domainfunction^{\textup{F}}}
\newcommand{\domainf}[2]{\domainffunction_{#1}}
\newcommand{\costswitch}{\varrho}
\newcommand{\costswitchf}[1]{\costswitch_{#1}}




\newcommand{\aralt}{\bar\ar}
\newcommand{\ewd}[1]{\exp{-{#1}\strate\st}}
\newcommand{\Kikl}[2]{K(#1,#2)}
\newcommand{\hypergeometricfunction}{\tensor[_{\,2\!}]{F}{_1}}
\newcommand{\hypergeometric}[4]{\hypergeometricfunction(#1,#2;#3;#4)}
\newcommand{\laguerrepolynomial}[1]{L_{#1}}
\newcommand{\laguerre}[2]{\laguerrepolynomial{#1}(#2)}
\newcommand{\Zlaguerrepolynomial}{Z}
\newcommand{\Zlaguerre}[3]{\Zlaguerrepolynomial_{#1}^{(#2)}(#3)}
\newcommand{\Deltalaguerrepolynomial}[1]{\laguerrepolynomial{#1}^{\Delta}}
\newcommand{\Deltalaguerre}[2]{\Deltalaguerrepolynomial{#1}(#2)}
\newcommand{\genlaguerrepolynomial}[2]{\laguerrepolynomial{#1}^{(#2)}}
\newcommand{\genlaguerre}[3]{\genlaguerrepolynomial{#1}{#2}(#3)}
\newcommand{\xiq}[1]{\xivar(#1)}
\newcommand{\xivar}{\mu}

\newcommand{\nbservers}{k}

\newcommand{\admissionoperator}{\mathcal{A}}
\newcommand{\admissionfoperator}[2]{\admissionoperator_{#1,#2}}
\newcommand{\admissionfxy}[4]{\admissionfoperator{#1}{#2}(#3,#4)}
\newcommand{\admissionioperator}[1]{\admissionoperator_{#1}}
\newcommand{\admissioniux}[3]{\admissionioperator{#1}(#2,#3)}
\newcommand{\admissionicoperator}[2]{\admissionioperator{#1}}%^{#2}}
\newcommand{\admissionicux}[4]{\admissionicoperator{#1}{#2}(#3,#4)}
\newcommand{\admissionicostoperator}[2]{\admissionioperator{#1;#2}}
\newcommand{\admissionicostux}[4]{\admissionicoperator{#1}{#2}(#3,#4)}

\newcommand{\admissionfunction}{a}
\newcommand{\admissionx}[1]{\admissionfunction(#1)}
\newcommand{\admissionxy}[2]{\admissionfunction(#1,#2)}
\newcommand{\admissionifunction}[1]{\admissionfunction_{#1}}
\newcommand{\admissionix}[2]{\admissionifunction{#1}(#2)}
\newcommand{\admissionixy}[3]{\admissionifunction{#1}(#2,#3)}
\newcommand{\admissioncfunction}[1]{\makeclass{\admissionfunction}{#1}}
\newcommand{\admissioncx}[2]{\admissioncfunction{#1}(#2)}
\newcommand{\admissioncxcost}[3]{\admissioncfunction{#1}(#2,#3)}
\newcommand{\admissioncsfunction}[2]{\makeclassserver{\admissionfunction}{#1}{#2}}
\newcommand{\admissioncsx}[3]{\admissioncsfunction{#1}{#2}(#2)}
\newcommand{\admissioncsxcost}[4]{\admissioncsfunction{#1}{#2}(#3,#4)}
\newcommand{\intervadmissionicostux}[4]{\intervx{\admissionioperator{#1}}\left(#2;#3,#4\right)}

\newcommand{\probcs}[2]{\makeclassserver{\arprob}{#1}{#2}}

\newcommand{\Real}{\mathbb{R}}
\newcommand{\Realzero}{\Real_{0}}
\newcommand{\Realplus}{\Real_{>0}}
%\newcommand{\Realpluszero}{\Real_{\geq 0}}
\newcommand{\Realpluszero}{\Real_{\raisebox{0.5pt}{\tiny$\geq$} 0}}
\newcommand{\Realminus}{\Real_{<0}}
\newcommand{\Realminuszero}{\Real_{\leq 0}}
\newcommand{\Complex}{\mathbb{C}}
\newcommand{\Complexzero}{\Complex_0}
\newcommand{\Integer}{\mathbb{Z}}
\newcommand{\Integerzero}{\mathbb{Z}_0}
\newcommand{\Natural}{\mathbb{N}}
\newcommand{\Naturalzero}{\Natural_0}
\newcommand{\Naturalpos}{\Natural_{>0}}
\newcommand{\Naturalnn}{\Natural_{\geq 0}}
\newcommand{\Continuouslydifferentiable}{C}
\newcommand{\nContinuouslydifferentiable}[1]{\Continuouslydifferentiable^{#1}}


\newcommand{\complexexponent}[3]{{#1}^{#2}]_{#3}}
\newcommand{\Complexexponent}[3]{\left.{#1}^{#2}\right]_{#3}}
\newcommand{\textcomplexexponent}[3]{{#1}^{\scriptstyle{#2}}]_{#3}}
\newcommand{\complexarg}[2]{\arg {#1}]_{#2}}
\newcommand{\Complexarg}[2]{\left.\arg {#1}\right]_{#2}}
\newcommand{\complexsqrt}[2]{\sqrt{#1}]_{#2}}
\newcommand{\Complexsqrt}[2]{\left.{\sqrt{#1}}\,\right]_{#2}}

\newcommand{\tim}{t}
\newcommand{\Tim}{T}

\newcommand{\genericset}{\mathcal{S}}
\newcommand{\genericblset}{\mathcal{U}}
\newcommand{\genericstset}{\mathcal{X}}
\newcommand{\genericsequencefunction}{h}
\newcommand{\genericsequence}[1]{\genericsequencefunction[#1]}
\newcommand{\genericfunction}{f}
\newcommand{\Genericfunction}{F}
\newcommand{\genericfx}[1]{\Genericfunction({#1})}
\newcommand{\laplacegenerics}[1]{\Genericfunction({#1})}
\newcommand{\genericx}[1]{\genericfunction({#1})}
\newcommand{\altgenericfunction}{g}
\newcommand{\altgenericx}[1]{\altgenericfunction({#1})}
\newcommand{\altgenericifunction}[1]{\altgenericfunction_{#1}}
\newcommand{\altgenericix}[2]{\altgenericifunction{#1}({#2})}
\newcommand{\altgenericnfunction}[1]{\makenindex{\altgenericfunction}{#1}}
\newcommand{\altgenericnx}[2]{\altgenericnfunction{#1}(#2)}
\newcommand{\altgenericnifunction}[2]{\makenindex{\altgenericfunction}{#1}_{#2}}
\newcommand{\altgenericnix}[3]{\altgenericnifunction{#1}{#2}(#3)}


\newcommand{\zcomplex}{z}
%\newcommand{\Ztransformf}[1]{\mathcal{Z}(#1)}
\newcommand{\Ztransformf}[1]{\mathcal{Z}_{#1}}
\newcommand{\Ztransformfz}[2]{\Ztransformf{#1}(#2)}
%\newcommand{\inverseZtransformf}[1]{\mathcal{Z}^{-1}(#1)}
\newcommand{\inverseZtransformf}[1]{\mathcal{Z}^{-1}_{#1}}
\newcommand{\inverseZtransformfx}[2]{\inverseZtransformf{#1}(#2)}


%\newcommand{\realpart}[1]{\operatorname{Re}(#1)}
%\newcommand{\imaginarypart}[1]{\operatorname{Im}(#1)}
%\newcommand{\Realpart}[1]{\operatorname{Re}\left(#1\right)}
%\newcommand{\Imaginarypart}[1]{\operatorname{Im}\left(#1\right)}
\newcommand{\realpart}[1]{\Re(#1)}
\newcommand{\imaginarypart}[1]{\Im(#1)}
\newcommand{\Realpart}[1]{\Re\left(#1\right)}
\newcommand{\Imaginarypart}[1]{\Im\left(#1\right)}
\newcommand{\complex}{s}
\newcommand{\altcomplex}{\sigma}
%\newcommand{\laplacetransformf}[1]{\mathcal{L}(#1)}
\newcommand{\laplacetransformf}[1]{\mathcal{L}_{#1}}
\newcommand{\laplacetransformfs}[2]{\laplacetransformf{#1}(#2)}
%\newcommand{\inverselaplacetransformf}[1]{\mathcal{L}^{-1}(#1)}
\newcommand{\inverselaplacetransformf}[1]{\mathcal{L}^{-1}_{#1}}
\newcommand{\inverselaplacetransformfx}[2]{\inverselaplacetransformf{#1}(#2)}
\newcommand{\Blaplacetransformf}[1]{\mathcal{B}_{#1}}
\newcommand{\Blaplacetransformfs}[2]{\Blaplacetransformf{#1}(#2)}
\newcommand{\inverseBlaplacetransformf}[1]{\mathcal{B}^{-1}_{#1}}
\newcommand{\inverseBlaplacetransformfx}[2]{\inverseBlaplacetransformf{#1}(#2)}
\newcommand{\analyticpartfunction}{h}
\newcommand{\analyticparts}[1]{\analyticpartfunction(#1)}
\newcommand{\altanalyticpartfunction}{\tilde\analyticpartfunction}
\newcommand{\altanalyticparts}[1]{\altanalyticpartfunction(#1)}
\newcommand{\anticausalfunction}{r}
\newcommand{\anticausalx}[1]{\anticausalfunction(#1)}
\newcommand{\altanticausalfunction}{\tilde\anticausalfunction}
\newcommand{\altanticausalx}[1]{\altanticausalfunction(#1)}
\newcommand{\fr}{f}
\newcommand{\fouriertransformf}[1]{\mathcal{F}_{#1}}
\newcommand{\fouriertransformfomega}[2]{\fouriertransformf{#1}(#2)}
\newcommand{\fouriertransformff}[2]{\fouriertransformf{#1}(#2)}
\newcommand{\inversefouriertransformf}[1]{\mathcal{F}^{-1}_{#1}}
\newcommand{\inversefouriertransformfx}[2]{\inversefouriertransformf{#1}(#2)}
\newcommand{\laplacegenericfunction}{\mathcal{\Genericfunction}}
\newcommand{\laplacegenericfs}[1]{\laplacegenericfunction({#1})}
\newcommand{\laplacevaluefunction}{\mathcal{\Valuefunction}}
\newcommand{\laplacevalues}[1]{\laplacevaluefunction({#1})}
\newcommand{\laplaceboundvaluefunction}{\bar{\mathcal{\Valuefunction}}}
\newcommand{\laplaceboundvalues}[1]{\laplaceboundvaluefunction({#1})}
\newcommand{\laplacevaluezerofunction}{\mathcal{\Valuefunction}_0}
\newcommand{\laplacevaluezeros}[1]{\laplacevaluezerofunction(#1)}
\newcommand{\laplacecostfunction}{\mathcal{\costfunction}}
\newcommand{\laplacecosts}[1]{\laplacecostfunction({#1})}
\newcommand{\laplacestochcostfunction}{\mathcal{\stochcostfunction}}
\newcommand{\laplacestochcosts}[1]{\laplacestochcostfunction({#1})}
\newcommand{\laplacediffvaluefunction}{\tilde{\mathbb{Y}}}
\newcommand{\laplacediffvalueifunction}[1]{\laplacediffvaluefunction_{#1}}
\newcommand{\laplacediffvalueis}[2]{\laplacediffvalueifunction{#1}(#2)}
\newcommand{\laplacecutdiffvaluefunction}{\bar{\mathcal{Y}}}
\newcommand{\laplacecutdiffvalueifunction}[1]{\laplacecutdiffvaluefunction_{#1}}
\newcommand{\laplacecutdiffvalueis}[2]{\laplacecutdiffvalueifunction{#1}(#2)}
\newcommand{\laplacelaurentdiffvaluefunction}{\hat{\mathcal{Y}}}
\newcommand{\laplacelaurentdiffvalueifunction}[1]{\laplacelaurentdiffvaluefunction_{#1}}
\newcommand{\laplacelaurentdiffvalueis}[2]{\laplacelaurentdiffvalueifunction{#1}(#2)}
\newcommand{\laplaceshifteddiffvaluefunction}{\shifted{\mathcal{Y}}}
\newcommand{\laplaceshifteddiffvalueidfunction}[2]{\laplaceshifteddiffvaluefunction_{#1}^{[#2]}}
\newcommand{\laplaceshifteddiffvalueids}[3]{\laplaceshifteddiffvalueidfunction{#1}{#2}(#3)}
\newcommand{\contourfunction}{\mathcal{C}}
\newcommand{\arcfunction}{\mathcal{A}}
\newcommand{\contoura}[1]{\contourfunction_{#1}}
\newcommand{\contouras}[2]{\contoura{#1}(#2)}
\newcommand{\arca}[1]{\arcfunction_{#1}}
\newcommand{\laplaceshiftedvaluefunction}{\shifted{\mathcal{\Valuefunction}}}
\newcommand{\laplaceshiftedvaluedfunction}[1]{\laplaceshiftedvaluefunction^{[#1]}}
\newcommand{\laplaceshiftedvalueds}[2]{\laplaceshiftedvaluedfunction{#1}(#2)}




\newcommand{\vfclass}{\mathcal{M}}
\newcommand{\anchor}{\gamma}

\newcommand{\valueifunction}[1]{\valuefunction_{#1}}
\newcommand{\valueix}[2]{\valueifunction{#1}(#2)}
\newcommand{\purevalueifunction}[1]{\purevaluefunction_{#1}}
\newcommand{\purevalueix}[2]{\purevalueifunction{#1}(#2)}
\newcommand{\costratei}[1]{\costrate_{#1}}
\newcommand{\mean}[1]{\meancost_{#1}}
\newcommand{\costifunction}[1]{\costfunction_{#1}}
\newcommand{\costix}[2]{\costifunction{#1}(#2)}
\newcommand{\Costix}[2]{\costifunction{#1}\left(#2\right)}

\newcommand{\holom}[2]{\tilde{\mathcal{H}}_{#1}(#2)}
\newcommand{\ncoefzero}[1]{\alpha_{#1}}
\newcommand{\ncoefar}[2]{\beta_{#1}^{(#2)}}
\newcommand{\ncoefnew}[2]{\gamma_{#1}^{(#2)}}
\newcommand{\ncoefalt}[2]{\bar{\gamma}_{#1}^{(#2)}}
\newcommand{\shiftedncoefar}[2]{\shifted{\beta}_{#1}^{(#2)}}
\newcommand{\shiftedncoefarrandomst}[3]{\shifted{\beta}_{#1;#2}^{(#3)}}
\newcommand{\boundaryncoefar}[2]{{\gamma}_{#1}^{(#2)}}

\newcommand{\shifted}[1]{\overleftarrow{#1}}



\newcommand{\rootn}[1]{\complex^*_{#1}}


\newcommand{\singularity}{\hat\complex}
\newcommand{\singularityk}[1]{\singularity_{#1}}
\newcommand{\degreei}[1]{\zeta_{#1}}
\newcommand{\laurent}[1]{a_{#1}}
\newcommand{\lambertfunction}{W}
\newcommand{\lambertnfunction}[1]{\lambertfunction_{#1}}
\newcommand{\lambertnx}[2]{\lambertnfunction{#1}(#2)}
\newcommand{\Lambertnx}[2]{\lambertnfunction{#1}\left(#2\right)}
\newcommand{\lambertkfunction}[1]{\lambertfunction_{#1}}
\newcommand{\lambertkx}[2]{\lambertkfunction{#1}(#2)}
\newcommand{\residuefunction}{\textup{Res}}
%\newcommand{\Residuefx}[2]{\residuefunction\left(#1,#2\right)}
%\newcommand{\residuefx}[2]{\residuefunction(#1,#2)}
\newcommand{\Residuefx}[2]{\residuefunction_{#2}\left({#1}\right)}
\newcommand{\bigresiduefx}[2]{\residuefunction_{#2}\big({#1}\big)}
\newcommand{\Bigresiduefx}[2]{\residuefunction_{#2}\Big({#1}\Big)}
\newcommand{\biggresiduefx}[2]{\residuefunction_{#2}\bigg({#1}\bigg)}
\newcommand{\residuefx}[2]{\residuefunction_{#2}{#1}}
\newcommand{\residualfunction}{\textup{Res}}
\newcommand{\residual}[1]{\residualfunction(#1)}
\newcommand{\residualifunction}[1]{\residualfunction_{#1}}
\newcommand{\residualisx}[3]{\residualifunction{#1}(#2,#3)}
\newcommand{\residualfsx}[3]{\residualifunction{#1}(#2,#3)}
\newcommand{\Singularities}[1]{\textup{S}_{#1}}
\newcommand{\Singf}[1]{\textup{S}_{#1}}

\newcommand{\stochX}{X}
\newcommand{\stochN}{N}
\newcommand{\stochT}{T}
\newcommand{\stochsum}{S}
\newcommand{\stochXk}[1]{\stochX_{#1}}
\newcommand{\stochstj}[1]{\stochst_{#1}}
\newcommand{\stochstk}[1]{\stochst_{#1}}
\newcommand{\stochTk}[1]{\stochT_{#1}}
\newcommand{\stochNk}[1]{\stochN_{#1}}
\newcommand{\stochstkl}[2]{\stochst_{#1,#2}}
\newcommand{\stochsumk}[1]{\stochsum_{#1}}
\newcommand{\Numfunction}[1]{N_{#1}}
\newcommand{\Num}[2]{\Numfunction{#1}(#2)}
\newcommand{\Denfunction}{D}
\newcommand{\Den}[1]{\Denfunction(#1)}

\newcommand{\class}{l}
\newcommand{\altclass}{p}
\newcommand{\server}{i}
\newcommand{\altserver}{j}
\newcommand{\makeclass}[2]{{#1}^{\text{\tiny{$\lbrack{#2}\rbrack$}}}}
\newcommand{\makeserver}[2]{#1_{\text{\tiny{$\lbrack#2\rbrack$}}}}
%\newcommand{\makeclassserver}[3]{{#1}^{\text{\tiny{$(#2,#3)$}}}}
\newcommand{\makeclassserver}[3]{\makeserver{\makeclass{#1}{#2}}{#3}}

%\newcommand{\exp}[1]{e^{#1}}

\renewcommand{\Valuetfunction}[1]{\Valuefunction^{(#1)}}
\newcommand{\eqD}{\,{\buildrel d \over =}\,}
\newcommand{\limbrace}[2]{\lim_{#1}\{#2\}}
\newcommand{\limbracenolimits}[2]{\lim\nolimits_{#1}\{#2\}}
\newcommand{\limBrace}[2]{\lim_{#1}\left\{#2\right\}}
\newcommand{\limBracenolimits}[2]{\lim\nolimits_{#1}\left\{#2\right\}}
\newcommand{\toas}{\overset{a.s.}{\longrightarrow}}
\newcommand{\stochcostfunction}{C}
\newcommand{\altstochcostfunction}{\tilde\stochcostfunction}
\newcommand{\leftstochcostfunction}{\stochcostfunction^-}
\newcommand{\rightstochcostfunction}{\stochcostfunction^+}
\newcommand{\stochcostx}[1]{\stochcostfunction(#1)}
\newcommand{\altstochcostx}[1]{\altstochcostfunction(#1)}
\newcommand{\leftstochcostx}[1]{\leftstochcostfunction(#1)}
\newcommand{\rightstochcostx}[1]{\rightstochcostfunction(#1)}

\newcommand{\altcostfunction}{\tilde\costfunction}
\newcommand{\leftcostfunction}{\costfunction^-}
\newcommand{\rightcostfunction}{\costfunction^+}
\newcommand{\altcostx}[1]{\altcostfunction(#1)}
\newcommand{\leftcostx}[1]{\leftcostfunction(#1)}
\newcommand{\rightcostx}[1]{\rightcostfunction(#1)}

\renewcommand{\stochst}{D}
\renewcommand{\deltat}{\delta}

\newcommand{\todistribution}{\xrightarrow{d}}
\newcommand{\eqdistribution}{\overset{d}{=}}


\newcommand{\diffvaluefunction}{\tilde{y}}
\newcommand{\diffvalueifunction}[1]{\diffvaluefunction_{#1}}
\newcommand{\diffvalueix}[2]{\diffvalueifunction{#1}(#2)}
\newcommand{\diffvaluemufunction}[1]{\diffvaluefunction({#1},\cdot)}
\newcommand{\diffvaluemux}[2]{\diffvaluefunction({#1},#2)}
\newcommand{\ddiffvaluefunction}{\diffvaluefunction^{\prime}}
\newcommand{\ddiffvalueifunction}[1]{\ddiffvaluefunction_{#1}}
\newcommand{\ddiffvalueix}[2]{\ddiffvalueifunction{#1}(#2)}
\newcommand{\cutdiffvaluefunction}{\hat{y}}
\newcommand{\cutdiffvalueifunction}[1]{\cutdiffvaluefunction_{#1}}
\newcommand{\cutdiffvalueix}[2]{\cutdiffvalueifunction{#1}(#2)}
\newcommand{\shifteddiffvaluefunction}{\overleftarrow{y}}
\newcommand{\shifteddiffvalueidfunction}[2]{\shifteddiffvaluefunction_{#1}^{[#2]}}
\newcommand{\shifteddiffvalueidx}[3]{\shifteddiffvalueidfunction{#1}{#2}(#3)}
\newcommand{\shiftedvaluefunction}{\overleftarrow{\valuefunction}}
\newcommand{\shiftedvaluedfunction}[1]{\shiftedvaluefunction^{[#1]}}
\newcommand{\shiftedvaluedx}[2]{\shiftedvaluedfunction{#1}(#2)}
\newcommand{\shiftedpurevaluefunction}{\overleftarrow{\purevaluefunction}}
\newcommand{\shiftedpurevaluedfunction}[1]{\shiftedpurevaluefunction^{[#1]}}
\newcommand{\shiftedpurevaluedx}[2]{\shiftedpurevaluedfunction{#1}(#2)}
\newcommand{\shiftedgenericfunction}{\overleftarrow{\genericfunction}}
\newcommand{\shiftedgenericdfunction}[1]{\shiftedgenericfunction^{[#1]}}
\newcommand{\shiftedgenericdx}[2]{\shiftedgenericdfunction{#1}(#2)}
\newcommand{\cfunction}{c}
\newcommand{\cifunction}[1]{\cfunction_{#1}}
\newcommand{\cix}[2]{\cifunction{#1}(#2)}
\newcommand{\dcfunction}{\cfunction^{\prime}}
\newcommand{\dcifunction}[1]{\dcfunction_{#1}}
\newcommand{\dcix}[2]{\dcifunction{#1}(#2)}
\newcommand{\tildevaluefunction}{\tilde{\valuefunction}}
\newcommand{\tildevalueifunction}[1]{\tildevaluefunction_{#1}}
\newcommand{\tildevalueix}[2]{\tildevalueifunction{#1}(#2)}
\renewcommand{\exp}[1]{e^{#1}}
\newcommand{\factorial}[1]{{#1}!}
\newcommand{\somei}{k}
\newcommand{\zfunction}{z}
\newcommand{\zifunction}[1]{\zfunction_{#1}}
\newcommand{\zix}[2]{\zifunction{#1}(#2)}
\newcommand{\zaltfunction}{\bar\zfunction}
\newcommand{\zaltifunction}[1]{\zaltfunction_{#1}}
\newcommand{\zaltix}[2]{\zaltifunction{#1}(#2)}
\newcommand{\zcfunction}[1]{\zfunction^{(#1)}}
\newcommand{\zcifunction}[2]{\zcfunction{#1}_{#2}}
\newcommand{\zcix}[3]{\zcifunction{#1}{#2}(#3)}
\newcommand{\termi}[1]{C_{#1}}


\providecommand{\obsolete}[1]{}

\renewcommand{\cost}{h}
\renewcommand{\stochcostfunction}{H}

\newcommand{\trsp}{T}


\newcommand{\subjectto}{\textup{subject to}}
\newcommand{\minimize}[2]{\textup{minimize}_{#1}{#2}}
\newcommand{\vect}[1]{(#1)}
\newcommand{\Vect}[1]{\left(#1\right)}
%\newcommand{\matrix}[1]{\left(#1\right)}



\newcommand{\prob}{p}
\newcommand{\probk}[1]{\prob^{#1}}
\newcommand{\probmax}{\bar\prob}
\newcommand{\probi}[1]{\prob_{#1}}
\newcommand{\probmaxi}[1]{\probmax_{#1}}
\newcommand{\probt}[1]{\prob^{#1}}
\newcommand{\probit}[2]{\probi{#1}^{#2}}
\newcommand{\Prob}{P}
\newcommand{\Probi}[1]{\Prob_{#1}}
%\newcommand{\st}{d}
\newcommand{\sti}[1]{\st_{#1}}
%\newcommand{\ar}{\lambda}
\newcommand{\ns}{n}
\newcommand{\np}{c}
\newcommand{\functionfunction}{f}
\newcommand{\fx}[1]{\functionfunction(#1)}
\newcommand{\dfunction}{\functionfunction^\prime}
\newcommand{\dfx}[1]{\dfunction(#1)}
\newcommand{\dnfunction}[1]{\functionfunction^{(#1)}}
\newcommand{\dnfx}[2]{\dnfunction{#1}(#2)}
\newcommand{\functioni}[1]{\functionfunction_{#1}}
\newcommand{\fix}[2]{\functionfunctioni{#1}(#2)}
\newcommand{\gprob}{x}
\newcommand{\dv}{y}
\newcommand{\dvmin}{\bar\dv}
\newcommand{\dvmini}[1]{\dvmin_{#1}}
\newcommand{\dvk}[1]{\dv^{#1}}
\newcommand{\hatdvi}[1]{\hat \dv_{#1}}
\newcommand{\dualfunction}{g}
\newcommand{\dualprimefunction}{\dualfunction^\prime}
\newcommand{\dualprimeprimefunction}{\dualfunction^{\prime\prime}}
\newcommand{\dualy}[1]{\dualfunction(#1)}
\newcommand{\dualprimey}[1]{\dualprimefunction(#1)}
\newcommand{\dualprimeprimey}[1]{\dualprimeprimefunction(#1)}
\newcommand{\dualifunction}[1]{\dualfunction_{#1}}
\newcommand{\dualiy}[2]{\dualifunction{#1}(#2)}
\newcommand{\dualprimeifunction}[1]{\dualprimefunction_{#1}}
\newcommand{\dualprimeiy}[2]{\dualprimeifunction{#1}(#2)}
\newcommand{\dualprimeprimeifunction}[1]{\dualprimeprimefunction_{#1}}
\newcommand{\dualprimeprimeiy}[2]{\dualprimeprimeifunction{#1}(#2)}
\newcommand{\lagrangefunction}{l}
\newcommand{\lagrangexy}[2]{\lagrangefunction(#1,#2)}
\newcommand{\lagrangeifunction}[1]{\lagrangefunction_{#1}}
\newcommand{\lagrangeixy}[3]{\lagrangeifunction{#1}(#2,{#3})}
\newcommand{\solfunction}{\gprob^\star}
\newcommand{\sol}[1]{\sol(#1)}
\newcommand{\solifunction}[1]{\solfunction_{#1}}
\newcommand{\soli}[2]{\solifunction{#1}(#2)}
\newcommand{\linesearch}{\alpha}
\newcommand{\linesearchk}[1]{\linesearch^{#1}}
\newcommand{\linesearchleftright}{\linesearch_{\mp}}
\newcommand{\linesearchleftrightk}[1]{\linesearchleftright^{#1}}
\newcommand{\linesearchleft}{\linesearch_{-}}
\newcommand{\linesearchleftk}[1]{\linesearchleft^{#1}}
\newcommand{\linesearchright}{\linesearch_{+}}
\newcommand{\linesearchrightk}[1]{\linesearchright^{#1}}
\newcommand{\linesearchlr}{\linesearch_{\mp}}
\newcommand{\linesearchlrk}[1]{\linesearchlr^{#1}}
\newcommand{\step}{\beta}
\newcommand{\stepk}[1]{\step^{#1}}
\newcommand{\genset}{S}
\newcommand{\linearset}{T}
\newcommand{\setstronglyconvex}{\genset}
\newcommand{\setlinear}{\linearset}
\newcommand{\setzero}{\bar\genset}
\newcommand{\setdvmin}{\bar\linearset}
\newcommand{\setstronglyconvexy}[1]{\setstronglyconvex(#1)}
\newcommand{\setlineary}[1]{\setlinear(#1)}
\newcommand{\setzeroy}[1]{\setzero(#1)}
\newcommand{\setdvminy}[1]{\setdvmin(#1)}

\newcommand{\cardinality}[1]{|{#1}|}
\newcommand{\Cardinality}[1]{\left|{#1}\right|}
\newcommand{\REALone}{\mathbb{R}}
\newcommand{\Min}[2]{\min\left(#1,#2\right)}
\newcommand{\Max}[2]{\max\left(#1,#2\right)}
\newcommand{\stepfunction}{\theta}
\newcommand{\stepx}[1]{\stepfunction(#1)}
\newcommand{\Stepx}[1]{\stepfunction\left(#1\right)}
\newcommand{\stepminusfunction}{\stepfunction^{-}}
\newcommand{\stepminusx}[1]{\stepminusfunction(#1)}
\newcommand{\Stepminusx}[1]{\stepminusfunction\left(#1\right)}
\newcommand{\leftderivative}{\partial_{-}} 
\newcommand{\rightderivative}{\partial_{+}} 
\newcommand{\lrderivative}{\partial_{\mp}} 
\newcommand{\indicatorsign}{\mathbf{1}}%{\mathbbm{1}}%
\newcommand{\indicatorfunction}[1]{\indicatorsign_{#1}}
\newcommand{\indicator}[2]{\indicatorfunction{#1}(#2)}
\newcommand{\Indicator}[2]{\indicatorfunction{#1}\left(#2\right)}


%\providecommand{\refeq}[2]{\overset{\text{\tiny{#1}}}{#2}}
%\renewcommand{\refeq}[2]{\overset{\text{\tiny{#1}}}{#2}}

\newcommand{\refereq}[2]{\overset{\text{\tiny{#1}}}{#2}}



\newcommand{\nintervals}{n}
\renewcommand{\ns}{s}

\newcommand{\measure}{\mu}
\newcommand{\measurex}[1]{\measure(#1)}
\newcommand{\measurei}[1]{\mu_{#1}}
\newcommand{\measureix}[2]{\measurei{#1}(#2)}
\newcommand{\measureXfunction}[1]{\mu_{#1}}
\newcommand{\measureXx}[2]{\measureXfunction{#1}(#2)}

\newcommand{\tildebl}{\tilde\bl}

\newcommand{\altfunction}{g}
\newcommand{\altfx}[1]{\altfunction({#1})}
\newcommand{\altfnfunction}[1]{\altfunction^{({#1})}}
\newcommand{\altfnx}[2]{\altfnfunction{#1}({#2})}

\newcommand{\tildealtfunction}{\tilde\altfunction}
\newcommand{\tildealtfx}[1]{\tildealtfunction({#1})}
\newcommand{\tildealtfnfunction}[1]{\tildealtfunction^{({#1})}}
\newcommand{\tildealtfnx}[2]{\tildealtfnfunction{#1}({#2})}

\newcommand{\altaltfunction}{h}
\newcommand{\altaltfx}[1]{\altaltfunction({#1})}
\newcommand{\altaltfnfunction}[1]{\altaltfunction^{({#1})}}
\newcommand{\altaltfnx}[2]{\altaltfnfunction{#1}({#2})}

\newcommand{\rudinfunction}{g}
\newcommand{\rudinaltfunction}{h}
\newcommand{\rudinfunctionn}[1]{\rudinfunction_{#1}}
\newcommand{\rudinft}[1]{\rudinfunction({#1})}
\newcommand{\rudinaltft}[1]{\rudinaltfunction({#1})}
\newcommand{\rudinfnt}[2]{\rudinfunctionn{#1}({#2})}
\newcommand{\rudinfnx}[2]{\rudinfunctionn{#1}({#2})}
\newcommand{\rudinA}{h}
\newcommand{\rudinAn}[1]{\rudinA_{#1}}
\newcommand{\rudinE}{E}
\newcommand{\rudinx}{x^\star}
\newcommand{\rudint}{x}
\newcommand{\rudintmax}{\rudint_0}
\newcommand{\rudinn}{k}

\newcommand{\sing}{a}
\newcommand{\altsing}{b}
%\newcommand{\Sing}{\mathcal{A}}
%\newcommand{\newSing}{\bar{\mathcal{A}}}
\newcommand{\newSing}{\mathcal{P}}
\newcommand{\newSingzero}{\newSing_0}

\newcommand{\costsx}[2]{\costfunction(#1,#2)}
\newcommand{\alttim}{k}
\newcommand{\altTim}{K}
\newcommand{\makeROC}[1]{\textup{ROC:}\ \{\zcomplex\in\Complex\setst{#1}\}}
\newcommand{\mainsolution}{main solution}
\newcommand{\mainsolutions}{main solutions}
\newcommand{\Mainsolution}{Main solution}
\newcommand{\Mainsolutions}{Main solutions}
%\newcommand{\balancedvf}{balanced value function}
%\newcommand{\balancedvfs}{balanced value functions}
%\newcommand{\Balancedvf}{Balanced value function}
%\newcommand{\Balancedvfs}{Balanced value functions}

%\newcommand{\balancedvf}{BVF}
%\newcommand{\balancedvfs}{BVFs}
%\newcommand{\Balancedvf}{BVF}
%\newcommand{\Balancedvfs}{BVFs}

%\newcommand{\balancedvf}{discharge function}
%\newcommand{\balancedvfs}{discharge functions}
%\newcommand{\Balancedvf}{Discharge function}
%\newcommand{\Balancedvfs}{Discharge functions}
%\newcommand{\balancedvf}{drain function}
%\newcommand{\balancedvfs}{drain functions}
%\newcommand{\Balancedvf}{Drain function}
%\newcommand{\Balancedvfs}{Drain functions}
%\newcommand{\balancedvf}{\acl{wfunction}}
%\newcommand{\balancedvfs}{\aclp{wfunction}}
%\newcommand{\Balancedvf}{\Acl{wfunction}}
%\newcommand{\Balancedvfs}{\Aclp{wfunction}}
\newcommand{\towelch}[2]{#2}
\newcommand{\CtoR}[2]{#2}
\newcommand{\keybl}{\hat\bl}
%\section{Definition}
\newcommand{\generatorfunction}{g}
\newcommand{\generatorarsingx}[3]{\generatorfunction(#1,#2,#3)}
\newcommand{\boundcst}{\kappa}
\newcommand{\jumpfunction}{G}
\newcommand{\jumptfunction}[1]{\jumpfunction_{#1}}
\newcommand{\jumpxt}[2]{\jumptfunction{#2}(#1)}
\newcommand{\jumptnfunction}[2]{\jumpfunction_{#1}^{#2}}
\newcommand{\jumpxtn}[3]{\jumptnfunction{#2}{#3}(#1)}
\newcommand{\jumpcostfunction}{C}
\newcommand{\jumpcosttfunction}[1]{\jumpcostfunction_{#1}}
\newcommand{\jumpcostxt}[2]{\jumpcosttfunction{#2}(#1)}
\newcommand{\jumpcostx}[1]{\jumpcostfunction(#1)}
\newcommand{\eventA}{A}
\newcommand{\eventB}{B}
\newcommand{\nstep}{n}
\newcommand{\vfconstantfunction}{K}
\newcommand{\vfconstantv}[1]{\vfconstantfunction_{#1}}
\newcommand{\dvzero}{g_0}
\newcommand{\hatbl}{\hat{U}}
\newcommand{\previouscoeffunction}{g}
\newcommand{\previouscoeftar}[2]{\previouscoeffunction(#1,#2)}
\newcommand{\polecst}{a}
\newcommand{\extpole}{\eta}
\newcommand{\cstone}{\kappa_1}
\newcommand{\csttwo}{\kappa_2}
\newcommand{\cstB}{b}
\newcommand{\cstbarb}{\bar\scaledremfunction}
\newcommand{\cstD}{\Delta}
\newcommand{\csteps}{\upsilon}
\newcommand{\remfunction}{g}
\newcommand{\remx}[1]{\remfunction(#1)}
\newcommand{\scaledremfunction}{h}
\newcommand{\scaledremx}[1]{\scaledremfunction(#1)}
\newcommand{\contrfunction}{f}
\newcommand{\contrfxy}[2]{\contrfunction(#1,#2)}
\newcommand{\contrcstone}{b}
\newcommand{\contrbndone}{b_1}
\newcommand{\contrbndtwo}{b_2}
\newcommand{\contrbndthree}{b_3}
%%%%%%
\newcommand{\sumfunction}{\chi}
\newcommand{\sumx}[1]{\sumfunction(#1)}
\newcommand{\sumsumfunction}{\psi}
\newcommand{\sumsumx}[1]{\sumsumfunction(#1)}
\newcommand{\csumfunction}{\tilde{\sumfunction}}
\newcommand{\csumx}[1]{\csumfunction(#1)}
\newcommand{\csumsumfunction}{\tilde{\sumsumfunction}}
\newcommand{\csumsumx}[1]{\csumsumfunction(#1)}
\newcommand{\eorder}{\varrho}
\newcommand{\etype}{\sigma}
\newcommand{\boundvdfunction}{\beta}
\newcommand{\boundvdk}[1]{\boundvdfunction_{#1}}
\newcommand{\sspn}[1]{l_{#1}}
\newcommand{\ssqn}[1]{m_{#1}}
%
\newcommand{\radius}{r}
\newcommand{\phase}{\alpha}
\newcommand{\degree}[1]{\Delta({#1})}
%\newcommand{\orderfs}[2]{n_{#1}({#2})}
%\newcommand{\orderfs}[2]{\eta({#2})}%{\dot{n}({#2})}
\newcommand{\orderfs}[2]{\eta_{#2}}%{\dot{n}({#2})}
\newcommand{\remainderifunction}[1]{R_{#1}}
\newcommand{\remainderis}[2]{\remainderifunction{#1}(#2)}
\newcommand{\aCfunction}{\chi}
\newcommand{\aCarsing}[2]{\aCfunction(#1,#2)}
\newcommand{\Cfunction}{\psi}
\newcommand{\Carsing}[2]{\Cfunction(#1,#2)}
\newcommand{\primaCnfunction}[1]{\tilde\chi^{(#1)}}
\newcommand{\primaCnarsing}[3]{\primaCnfunction{#1}(#2,#3)}
\newcommand{\sqprimaCnfunction}[1]{\tilde\varphi^{(#1)}}
\newcommand{\sqprimaCnarsing}[3]{\sqprimaCnfunction{#1}(#2,#3)}
\newcommand{\Atermt}[1]{A^{(#1)}}
\newcommand{\Aterm}[1]{A(#1)}
\newcommand{\Bterm}[1]{B(#1)}
\newcommand{\sthreshold}{\varrho}
\newcommand{\ncycle}{\bar{n}}
%
\newcommand{\rone}{2}
\newcommand{\rtwo}{1}
\newcommand{\rthree}{5}
\newcommand{\rfour}{\dddjcdn}
\newcommand{\rfive}{3}
\newcommand{\rsix}{4}
\newcommand{\rseven}{6}
\newcommand{\reight}{7}
%
\newcommand{\nn}{n}
%
\newcommand{\identityn}[1]{I^{(#1)}}
\newcommand{\uppertriangularn}[1]{\uppertriangular^{(#1)}}
\newcommand{\strictlyuppertriangularn}[1]{\tilde{M}^{(#1)}}
\newcommand{\Atermvectorn}[1]{w^{(#1)}}
\newcommand{\constantvectorn}[1]{p^{(#1)}}
\newcommand{\complexvectorn}[1]{y^{(#1)}}
%\newcommand{\specialmatrixfunction}{z}
%\newcommand{\specialmatrix}{Z}
\newcommand{\specialmatrixn}[1]{\specialmatrix^{(#1)}}
%\newcommand{\specialmatrixnk}[2]{z^{(#1)}_{#2}}
\newcommand{\specialmatrixnk}[2]{\specialmatrixfunction_{#2}}
\newcommand{\relativespecialmatrixnk}[2]{\bar{\specialmatrixfunction}_{#2}}
\newcommand{\specialmatrixnij}[3]{\specialmatrixn{#1}_{#2,#3}}
\newcommand{\uppervectorn}[1]{q^{(#1)}}
\newcommand{\revuppervectorn}[1]{r^{(#1)}}
\newcommand{\diffuppervectornk}[2]{\Delta^{(#1)}_{(#2)}}
\newcommand{\agr}{\varrho}%{\kappa}
\newcommand{\metoe}[2]{#2}%{{#1}:{#2}}
%%%
\newcommand{\sdmeancost}{\hat\costfunction}
\newcommand{\sdvaluefunction}{\hat\valuefunction}
\newcommand{\dsdvaluefunction}{\sdvaluefunction^\prime}
\newcommand{\ddsdvaluefunction}{\svaluefunction^{\prime\prime}}
\newcommand{\sdvaluex}[1]{\sdvaluefunction(#1)}
\newcommand{\dsdvaluex}[1]{\dsdvaluefunction(#1)}
\newcommand{\ddsdvaluex}[1]{\ddsdvaluefunction(#1)}
%
\newcommand{\UN}{M}
\newcommand{\YN}{N}
\newcommand{\totN}{N}
\newcommand{\NUi}[1]{\UN_{#1}}
\newcommand{\NY}{\YN}
\newcommand{\Ntot}{\totN}
\newcommand{\tUwt}{U}%{\tilde{\Uwt}}
\newcommand{\tUwtij}[2]{\tUwt_{#1#2}}
\newcommand{\Uwt}{Z}%{U}
\newcommand{\Uwtij}[2]{\Uwt_{#1#2}}
\newcommand{\Ywt}{Y}
\newcommand{\Ywti}[1]{\Ywt_{#1}}
%
\newcommand{\indexstyle}[1]{\textup{\scalebox{0.8}{$(#1)$}}}
%\newcommand{\indexstyle}[1]{(#1)}
\newcommand{\tUwtk}[1]{\tUwt^{\indexstyle{#1}}}
\newcommand{\tUwtijk}[3]{\tUwtk{#3}_{#1#2}}
\newcommand{\NUk}[1]{\UN^{\indexstyle{#1}}}
\newcommand{\NUik}[2]{\NUk{#2}_{#1}}
\newcommand{\Uwtk}[1]{\Uwt^{\indexstyle{#1}}}
\newcommand{\Uwtijk}[3]{\Uwtk{#3}_{#1#2}}
\newcommand{\Ywtk}[1]{\Ywt^{\indexstyle{#1}}}
\newcommand{\Ywtik}[2]{\Ywtk{#2}_{#1}}
\newcommand{\NYk}[1]{\YN^{\indexstyle{#1}}}
\newcommand{\Ntotk}[1]{\totN^{\indexstyle{#1}}}
\newcommand{\stochstij}[2]{\stochst_{#1}}
%\newcommand{\stochT}{T}
\newcommand{\stochTi}[1]{\stochT_{#1}}
%
\newcommand{\cumul}{\Psi}
\newcommand{\cumulfunction}{\cumul}
\newcommand{\cumulSfunction}[1]{\cumulfunction_{#1}}
\newcommand{\cumulSx}[2]{\cumulSfunction{#1}(#2)}
\newcommand{\dcumulfunction}{\cumulfunction^{\prime}}
\newcommand{\dcumulSfunction}[1]{\dcumulfunction_{#1}}
\newcommand{\dcumulSx}[2]{\dcumulSfunction{#1}(#2)}
\newcommand{\genS}{S}
%\newcommand{\Sone}{A}
%\newcommand{\Stwoi}[1]{B_{#1}}
%\newcommand{\Sthree}{C}
\newcommand{\Sone}{C}
\newcommand{\Stwoi}[1]{A_{#1}}
\newcommand{\Sthree}{B}
%
\newcommand{\sdcoeffunction}{\phi}
\newcommand{\sdcoef}[1]{\sdcoeffunction({#1})}
\newcommand{\vfshift}{\sdcoeffunction}
%
\newcommand{\switchc}{c^{(s)}}
\newcommand{\switchst}{d^{(s)}}
\newcommand{\strictlyornot}[2]{{#2}}
\newcommand{\coefvector}{a}
\newcommand{\coefn}[1]{\coefvector_{#1}}
\newcommand{\redefinez}[2]{#2}%{#1 --- #2}
\newcommand{\fixsign}[2]{#2}%{[{#1}\rightarrow{#2}]}
\newcommand{\freq}{f}
\newcommand{\phasespeed}{\omega}
%





\newcommand{\powcoeffunction}{\specialmatrixfunction}%{y}%{y_{#1}}
\newcommand{\powacoeffunction}[1]{\prescript{}{#1}{\powcoeffunction}}%{y_{#1}}
%\newcommand{\powacoefnk}[3]{\powacoeffunction{#1}^{(#2)}_{#3}} %{\powacoeffunction{#1}^{(#2)}[#3]}
%\newcommand{\poweracoefnk}[3]{\powacoeffunction{#1}_{#3}}%{\powacoeffunction{#1}[#3]}
\newcommand{\powacoefnk}[3]{\powcoeffunction_{{#1}:{#3}}^{(#2)}} %{\powacoeffunction{#1}^{(#2)}[#3]}
\newcommand{\poweracoefnk}[3]{\powcoeffunction_{{#1}:{#3}}}%{\powacoeffunction{#1}[#3]}

\newcommand{\powzeroXcoeffunction}{x}
\newcommand{\powaXcoeffunction}[1]{\prescript{}{#1}{\powzeroXcoeffunction}}
\newcommand{\powerzeroXcoefnk}[1]{\powzeroXcoeffunction_{#1}}
%\newcommand{\poweraXcoefnk}[2]{\powaXcoeffunction{#1}_{#2}}
\newcommand{\poweraXcoefnk}[2]{\powzeroXcoeffunction_{#1:#2}}

\newcommand{\makesquare}[7]{%
\fill[#7] (#1-#3,#2-#4) rectangle (#1+#3,#2+#4);
%	\fill[#6,opacity=1/5] (#1-#3+#5*#3*1/5,#2-#4+#5*#4*1/5) rectangle (#1+#3-#5*#3*1/5,#2+#4-#5*#4*1/5);
%	\fill[#6,opacity=2/5] (#1-#3+#5*#3*2/5,#2-#4+#5*#4*2/5) rectangle (#1+#3-#5*#3*2/5,#2+#4-#5*#4*2/5);
%	\fill[#6,opacity=3/5] (#1-#3+#5*#3*3/5,#2-#4+#5*#4*3/5) rectangle (#1+#3-#5*#3*3/5,#2+#4-#5*#4*3/5);
%	\fill[#6,opacity=4/5] (#1-#3+#5*#3*4/5,#2-#4+#5*#4*4/5) rectangle (#1+#3-#5*#3*4/5,#2+#4-#5*#4*4/5);
%	\fill[#6,opacity=5/5] (#1-#3+#5*#3*5/5,#2-#4+#5*#4*5/5) rectangle (#1+#3-#5*#3*5/5,#2+#4-#5*#4*5/5);
%\foreach \i in {0,...,\fn}
%	\fill[#6,opacity=\i/\fn] (#1-#3+#5*#3*\i/\fn,#2-#4+#5*#4*\i/\fn) rectangle (#1+#3-#5*#3*\i/\fn,#2+#4-#5*#4*\i/\fn);
\fill[#6!25!#7] (#1-#3+#5*#3*1/4,#2-#4+#5*#4*1/4) rectangle (#1+#3-#5*#3*1/4,#2+#4-#5*#4*1/4);
\fill[#6!50!#7] (#1-#3+#5*#3*2/4,#2-#4+#5*#4*2/4) rectangle (#1+#3-#5*#3*2/4,#2+#4-#5*#4*2/4);
\fill[#6!75!#7] (#1-#3+#5*#3*3/4,#2-#4+#5*#4*3/4) rectangle (#1+#3-#5*#3*3/4,#2+#4-#5*#4*3/4);
\fill[#6] (#1-#3+#5*#3,#2-#4+#5*#4) rectangle (#1+#3-#5*#3,#2+#4-#5*#4);
%
%\fill[#6] (#1-#3,#2-#4) rectangle (#1+#3,#2+#4);
%\fill[#7,path fading=fade bottom]  (#1-#3,#2-#4) rectangle (#1+#3,#2-#4+#5*#4);
%\fill[#7,path fading=fade top]  (#1-#3,#2+#4) rectangle (#1+#3,#2+#4-#5*#4);
%\fill[#7,path fading=fade left]  (#1-#3,#2-#4) rectangle (#1-#3+#5*#3,#2+#4);
%\fill[#7,path fading=fade right]  (#1+#3,#2-#4) rectangle (#1+#3-#5*#3,#2+#4);
}

